ARC: Alignment-based Redirection Controller for Redirected Walking in Complex Environments

We present a novel redirected walking controller based on alignment that allows the user to explore large and complex virtual environments, while minimizing the number of collisions with obstacles in the physical environment. Our alignment-based redirection controller, ARC, steers the user such that their proximity to obstacles in the physical environment matches the proximity to obstacles in the virtual environment as closely as possible. To quantify a controller's performance in complex environments, we introduce a new metric, Complexity Ratio (CR), to measure the relative environment complexity and characterize the difference in navigational complexity between the physical and virtual environments. Through extensive simulation-based experiments, we show that ARC significantly outperforms current state-of-the-art controllers in its ability to steer the user on a collision-free path. We also show through quantitative and qualitative measures of performance that our controller is robust in complex environments with many obstacles. Our method is applicable to arbitrary environments and operates without any user input or parameter tweaking, aside from the layout of the environments. We have implemented our algorithm on the Oculus Quest head-mounted display and evaluated its performance in environments with varying complexity. Our project website is available at https://gamma.umd.edu/arc/.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> alignment.tex <==
\section{Redirection by Alignment} \label{alignment}
The concept of alignment in the context of redirected walking was first formally studied by Thomas et al. \cite{thomas2020reactive}.
It should be noted, however, that key elements of alignment have been used in other RDW controllers prior to the work of Thomas et al. \cite{zmuda2013optimizing}.
That is, ideas that are fundamental components of alignment have been used in previous work on RDW controllers, but so far there is only one study that is concerned with understanding alignment during redirection explicitly as a formal idea \cite{thomas2020reactive}.
The present study is, to the best of our knowledge, the only other work that investigates redirection by alignment.
This section provides a definition of alignment that extends the definition introduced by Thomas et al. \cite{thomas2020reactive} to apply to arbitrary environments.
We also provide the details of our general alignment controller, for which the implementation is different from that of \cite{thomas2020reactive} in order to allow the algorithm to work without developer input in non-empty virtual environments.
\textbf{[NEED TO TALK ABOUT ONE OF THE ASSUMPTIONS OF REDIRECTION BY ALIGNMENT: WE ASSUME THAT THE USER WILL NOT WALK ON A VIRTUAL PATH THAT INCURS A COLLISION. This is very important to mention!! we also assume that the user only walks in the direction of their heading.]}

\subsection{Definitions and Background}
\subsubsection{Alignment}
\label{alignment-definition}
\textit{Alignment} is a configuration during which the user's physical state matches their virtual state, relative to nearby obstacles in the physical and virtual environments.
When this state is achieved, we say that the system (or user) is \textit{aligned}.
In general, a user's state can be described by different features depending on the use-case and the amount of detail needed.
It is up to the system developers to determine the state description that best encapsulates the alignment they want to achieve.
For the purposes of RDW, it is common to describe the user's state as their position and orientation in the physical and virtual environments.
This state description works well for achieving the alignment we desire (similar positions relative to obstacles) and is the description we use in the present study.

Formally, the state of the system is the union of physical and virtual states of the user in each environment:
\begin{equation}
\label{eqn:state}
    Q_t = \{ q_t^{physical}, q_t^{virtual} \},
\end{equation}
where $q_t^{physical}$ is the user's physical state at time $t$, $q_t^{virtual}$ is the user's virtual state at time $t$, and $Q_t$ is the union of both states at time $t$.
Note that $q_t^{physical}$ is in the explorable space of the physical environment, and $q_t^{virtual}$ is in the explorable space of the virtual environment, so $Q_t \in C_{free}$, where $C_{free}$ is the union of the physical and virtual free spaces.

Given $Q_t$, we can measure the alignment of the state by computing the distance between the physical and virtual states:
\begin{equation}
    A(Q_t) = dist(q_t^{physical}, q_t^{virtual}).
\end{equation}
The definition of $A(Q_t)$ has intentionally been left ambiguous, since the definition of alignment that we are providing is meant to be broadly applicable to a variety of situations and use-cases.
Thus, the exact definition of $dist(q_t^{physical}, q_t^{virtual})$ is determined by the developers and is dependent on the information stored in $q_t^{physical}$ and $q_t^{virtual}$, as well as the conditions necessary to achieve alignment (as determined by the developers).
For example, suppose we want to measure the alignment of a user's physical and virtual positions.
A reasonable definition of $q_t^{physical}$ and $q_t^{virtual}$ would be the user's physical and virtual positions, and we could define $dist(q_t^{physical}, q_t^{virtual})$ as the Euclidean distance.
It may also be the case that one value is not enough to accurately describe a user's degree of alignment.
In such a situation, $A(Q_t)$ can be a tuple of values, each of which describes one aspect of the alignment being measured.
% This is the case in the present paper, wherein we want to measure the similarity between the user's position \textit{and} orientation in the physical and virtual spaces (see \autoref{subsec:alignment-controller} for more details).

With traditional redirected walking controllers, the goal of the system is to steer the user away from obstacles in the physical environment.
With an alignment-based controller, the goal is to steer the user to a physical state that most closely matches the virtual state.
In general, the VE will differ greatly from the PE, so it is common that a particular virtual state does not have a physical state that it perfectly aligns with.
Thus, an alignment-based RDW controller aims to minimize the difference between the physical and virtual states (as defined by $A(Q_t)$), and does \textit{not} necessarily aim to perfectly align the two.
This inability to perfectly align the user is inherent to the size and configuration of obstacles in the VE and PE. 
Just as it is not reasonable to expect existing RDW controllers to be able to guarantee a collision-free experience in large, unconstrained VEs (as is commonly the case with traditional RDW controllers), it is not reasonable to expect a user to always be perfectly aligned at all times in complex VEs.
This means that there are different degrees of alignment: a user can be perfectly aligned, and they can also very misaligned.
% The degree of alignment depends on the state description we use and the metric we use to compare states.
It should be noted that if it were possible to keep a user aligned at all times, they would never encounter collisions while exploring a VE, and the virtual locomotion problem would be solved.

\subsubsection{Environment Complexity}
% complexity of environment
% env a:  
% 	- phys: 4.85685
% 	- virt: 4.85685
% 	- ratio: 1
% env b: 
% 	- phys: 3.09482
% 	- virt: 3.5926
% 	- ratio: 0.861443
% env c: 
% 	- phys: 3.39798
% 	- virt: 6.04238
% 	- ratio: 0.562358
The complexity of an environment is dependent on the task to be completed in said environment.
Thus, there is no single definition of complexity that can be used for all tasks \cite{crandall2003towards}.
In the context of navigation, environment complexity measures how difficult it is to navigate through an environment without colliding with any obstacles.
As the environment becomes populated with more obstacles, this navigation task becomes more difficult, and so the complexity of the environment increases.
Therefore, our definition of complexity should assign a high complexity to environments in which collision-free navigation is difficult.

For VR locomotion, the task is to move through a virtual environment without colliding with obstacles in the PE or VE.
We can describe the ease of avoiding collisions along a path using the distance to obstacles for all points along the path.
Extending this to the entire environment, we define environment complexity as the average distance to obstacles in all directions around the user, averaged across the entire free space of the environment.

Let $d(p, \theta)$ be the distance to the closest obstacle in the direction $\theta$ originating from a location $p = (x,y)$ in an environment.
This distance can be determined through simple ray-intersection queries.
We can measure the complexity at a point, denoted $\mathcal{C}(p)$, in an environment as the average distance to obstacles in all directions around $p$:
\begin{equation}
    \mathcal{C}(p) = \frac{1}{2\pi}\int_{0}^{2\pi}d(p, x)dx.
\end{equation}
See \autoref{fig:complexity} for an illustration of this definition.
To measure the complexity of the entire environment, denoted $\mathcal{C}(E)$, we compute the average complexity for all points in the environment $E$:
\begin{equation}
\label{eqn:env-complexity}
    \mathcal{C}(E) = \frac{1}{|P|}\sum_{p\in P}^{}\mathcal{C}(p),
\end{equation}
where $P$ is the set of all points $p$ in $E$.
When there is a lot of open space in an environment, $\mathcal{C}(E)$ will be large.
Conversely, $\mathcal{C}(E)$ approaches $0$ as the amount of open space in the environment decreases.

\begin{figure}[t]
    \centering
    \includegraphics[width=.25\textwidth]{img/complexity.png}
    \caption{A simplified view of  the ray-shooting queries that are computed to determine the complexity at a point. The point $p$ is shown as an orange circle, and the measurements to the closest obstacle in directions around $p$ are shown as blue dashed arrows. We show only twelve arrows in order to reduce visual clutter, but actual complexity computations should sample more rays.}
    \label{fig:complexity}
\end{figure}

Since VR locomotion involves both a physical and virtual environment, we must relate the environments' complexity measurements together.
To do this, we compute the \textit{complexity ratio} (CR) of the physical environment $E_{phys}$ and virtual environment $E_{virt}$:
\begin{equation}
    \text{CR} = \frac{E_{phys}}{E_{virt}}.
\end{equation}
This definition of environment complexity gives us an intuitive way to describe how easy it is to locomote through an environment, and the complexity ratio tells us how similar the complexities of two environments are.
As is typical in VR applications, when there is less space for locomotion in the PE than the VE, $\mathcal{C}(E_{phys}) < \mathcal{C}(E_{virt})$ and the complexity ratio will be between $0$ and $1$.
A value closer to 0 indicates a larger complexity disparity, which implies that a redirection controller will have a more difficult time avoiding collisions.

This definition for environment complexity operates on a continuous domain, which makes it difficult to compute.
To simplify the computation, we discretize the equation by sampling a point every $0.5$ meters in the environment, and sampling directions around $p$ in increments of $1^\circ$.

\subsection{Alignment-based Redirection Controller}
\label{subsec:alignment-controller}
% say something like "our controller needs to choose the appropriate gains at every frame in order to achieve or maintain alignment". just give the simple intro/overview of what the alignment-based controller is.
An overview of our controller can be seen in \autoref{fig:system_overview}.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/system_overview.png}
    \caption{An overview of the ARC redirection system for one frame. The input to the controller is the system state (physical and virtual user and environment states). ARC outputs rotation, translation, and curvature gains to be applied on the next frame based on how close the user is to alignment on the current frame.}
    \label{fig:system_overview}
\end{figure}

\subsubsection{Redirection Heuristic}
% - first need to define q_t^{physical} and q_t^{virtual}
% - then define  $dist(q_t^{physical}, q_t^{virtual})$
% - then define the gain selection heuristic
As mentioned in \autoref{alignment-definition}, is up to the developer to define the exact notions of state and alignment according to their use-case.
In this paper, we are concerned with creating a RDW controller that minimizes the number of collisions in complex environments.
The user's position and orientation in the environment is known at all times through the tracking information.
We define the user's state in the physical or virtual environment as the distance to the closest object in the environment, directly in front of the user and directly to the left and right of the user.
Formally, we define the user's physical state as:
\begin{equation}
    q_t^{physical} = \{ d(p_{phys}, \theta), d(p_{phys}, \theta+90^\circ), d(p_{phys}, \theta-90^\circ) \},
\end{equation}
where $p_{phys}$ is the user's position in the PE, $d(p_{phys}, \theta)$ is the distance to the closest physical object in the user's heading direction, $d(p_{phys}, \theta+90^\circ)$ is the distance to the closest physical object to the left of the user, and $d(p_{phys}, \theta-90^\circ)$ is the distance to the closest physical object to the right of the user.
We define $q_t^{virtual}$ in a similar manner, with the only difference being that we measure the distance to virtual objects relative to the user's virtual position and heading.
Knowing $q_t^{physical}$ and $q_t^{virtual}$, we can compute $Q_t$ as in \autoref{eqn:state}.
This definition of $Q_t$ is illustrated in \autoref{fig:state}.

\begin{figure}[t]
    \centering
    \includegraphics[width=.47\textwidth]{img/state.png}
    \caption{Visualization of the six values that constitute a user's state.}
    \label{fig:state}
\end{figure}

Given the definition of $q_t^{physical}$ and $q_t^{virtual}$, we can now compute $dist(q_t^{physical}, q_t^{virtual})$ so that we can quantify the alignment of a state.
We define the alignment distance function as:
\begin{equation}
    \begin{aligned}
    dist(q_t^{physical}, q_t^{virtual}) &= 
            | d(p_{phys}, \theta) - d(p_{virt}, \theta) | \\
            & + \ | d(p_{phys}, \theta+90^\circ) - d(p_{virt}, \theta+90^\circ) | \\
            & + \ | d(p_{phys}, \theta-90^\circ) - d(p_{virt}, \theta-90^\circ) |.
    \end{aligned}
\end{equation}
% \begin{equation}
%     \begin{aligned}
%     dist(q_t^{physical}, q_t^{virtual}) &= 
%             | d_{forward}^{physical} - d_{forward}^{virtual} | \\
%             & + \ | d_{left}^{physical} - d_{left}^{virtual} | \\
%             & + \ | d_{right}^{physical} - d_{right}^{virtual} |
%     \end{aligned}
% \end{equation}
% Given $A(Q_t)$, our controller now needs to determine the redirection gains to apply in order to minimize the alignment.
If $A(Q_t) = 0$, the system is perfectly aligned and no redirection gains are applied.
However, if $A(Q_t) \neq 0$, our controller uses heuristics that we defined in order to set the redirection gains.

If the user is translating, the translation gain $g_{trans}$ is set to be:
\begin{equation}
    g_{trans} = \text{clamp}\left(\frac{d(p_{phys}, \theta)}{d(p_{virt}, \theta)},\ minTransGain,\ maxTransGain\right).
\end{equation}
% \begin{equation}
%     g_{trans} = \text{clamp}\left(\frac{d_{forward}^{physical}}{d_{forward}^{virtual}},\ minTransGain,\ maxTransGain\right)
% \end{equation}
This heuristic speeds up the user's physical walking speed relative to their virtual walking speed if there is more open space in front of the physical user than there is in front of the virtual user.
% the closest physical obstacle in front is further away than the closest virtual obstacle in front.
If, instead, there is more space in front of the virtual user than there is in front of the physical user, the user's physical walking speed is slowed down relative to their virtual walking speed.
% the closest obstacle in front of the user in the PE is closer than in the VE, the user's physical walking speed is instead slowed down relative to their virtual walking speed.
We set $g_{trans}$ equal to the ratio of the distances, bounded by previous measured perceptual thresholds, so that the translation gain changes gradually, which increases user comfort.

Also if the user is translating, we need to set the curvature gain $g_{curve}$.
First, we determine which of the spaces to the left and the right of the physical user is more dissimilar to its virtual counterpart:
% First we determine if the space to the left or the right of the user is more misaligned:
\begin{equation}
    \begin{aligned}
    misalignLeft &= d(p_{phys}, \theta+90^\circ) - d(p_{virt}, \theta+90^\circ), \\
    misalignRight &= d(p_{phys}, \theta-90^\circ) - d(p_{virt}, \theta-90^\circ).
    \end{aligned}
\end{equation}
% \begin{equation}
%     \begin{aligned}
%     misalignLeft &= d_{left}^{physical} - d_{left}^{virtual} \\
%     misalignRight &= d_{right}^{physical} - d_{right}^{virtual} \\
%     \end{aligned}
% \end{equation}
If $misalignLeft > misalignRight$, we want to steer the user to the left in order to minimize the misalignment.
This is done by setting $g_{curve}$ as follows:
\begin{equation}\label{eqn:leftCurveGain}
    \begin{aligned}
    scalingFactor &= min(1, misalignLeft), \\
    g_{curve} &= min(1, scalingFactor \times maxCurvatureRadius).
    \end{aligned}
\end{equation}
If we instead want to steer the user to the right in order to minimize the misalignment (i.e. when $misalignRight > misalignLeft$), we set $g_{curve}$ in a similar manner to \autoref{eqn:leftCurveGain}, but we exchange $misalignLeft$ for $misalignRight$ in the $scalingFactor$ computation.
Similarly to the translation gain, we set $g_{curve}$ equal to the misalignment value, bounded by the curvature perceptual threshold, in order to smoothly transition between gains and reduce the jarring effects of that quickly change.
% If $misalignRight$ is equal to $misalignLeft$, we do not apply any curvature gain.

If the user is rotating, we set the gain according to the user's distance to objects in front of \textit{and} on both sides of the user.
Our heuristic for $g_{trans}$ only considered the distance to objects in front of the user, while the heuristic for $g_{curve}$ only considered the distances to objects on either side of the user.
However, our heuristic for the rotation gain considers all three distances in order to accurately describe the user's orientation.
Orientation is a function of all $360^\circ$ around the observer, so the most accurate measurement of orientational alignment would compare distances in all $360^\circ$ directions.
That degree of detail is not necessary to build an effective controller, since in actuality the distances will not usually not change very much over small changes in angle.
Furthermore, sampling distances in all direction around the observer is too computationally expensive to run in real-time, which is a requirement for reactive RDW controllers.

To set the rotation gain $g_{rota}$, we check if the direction that the user is turning is increasing or decreasing their rotational alignment.
To do this, we compare their rotational alignment in the current frame against their rotational alignment in the previous frame.
First, we compute the user's rotational alignment for the current and previous frames:
\begin{equation}\label{}
    \begin{aligned}
    curRotaAlignment &= dist(q_{t}^{physical}, q_{t}^{virtual}), \\
    prevRotaAlignment &= dist(q_{t-1}^{physical}, q_{t-1}^{virtual}).
    \end{aligned}
\end{equation}
Then, we set $g_{rota}$ according to if the current rotational alignment is better or worse than the previous rotational alignment:
\begin{equation}
    g_{trans} = 
    \begin{cases}
        minRotaGain & prevRotaAlignment < curRotaAlignment, \\
        maxRotaGain & prevRotaAlignment > curRotaAlignment, \\
        1 & \text{otherwise}.
    \end{cases}
\end{equation}
The intuition behind this heuristic is that we want to speed up the user's rotation when they are turning in a direction that improves their rotational alignment, and slow down their rotation when they are turning in a direction that worsens their rotational alignment.

\subsubsection{Resetting Heuristic}
Since we cannot guarantee that the user will travel on a collision-free physical path, our alignment-based controller needs a resetting policy to reorient the user when they are about to collide with a physical obstacle.
Our resetting policy is fairly simple: the user is reoriented to face the direction in the PE for which the distance to the closest physical object in the user's physical heading direction most closely matches the distance to the closest virtual object in the user's virtual heading direction.
One constraint on this resetting direction is that the direction the user faces after the reset must be facing away from the obstacle they collided with, to ensure that the do not continue to walk forward into the object.

Please refer to \autoref{fig:reset} for a visual explanation of our resetting heuristic.
When the user collides with an obstacle, the controller computes the distance to the closest physical obstacle in eight directions around the user, in increments of $45^\circ$.
Of these eight directions around the user, in order to ensure that the user faces away from the obstacle after resetting, we disregard any directions for which the dot product of the direction and the normal of the colliding obstacle's surface is less than 0.
Of the remaining valid directions, we find the direction for which the distance to the closest physical obstacle in that direction most closely matches the distance to the closest virtual obstacle in the direction of the user's current virtual heading.

Once the best direction is found, we turn the user to face that direction.
The user turns is instructed to place until they are aligned with the best direction of the eight sampled directions, while the virtual turn is scaled up to be a $360^\circ$ turn.
The user's turn is in the direction of the larger of the two angles between the user's heading before the reset and the desired heading after the reset.
This is done to minimize the amount of rotational distortion required for the turn, and is inspired by the reset method used by Bachmann et al. \cite{bachmann2019multi}.

\begin{figure}[]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \includegraphics[width=\textwidth]{img/reset1_labeled.png}
        \caption{Selecting the best resetting direction. Invalid directions that cause the user to face the obstacle are colored in red. The best direction (pointing straight up) for resetting is highlighted, while the other directions are shown with a lower opacity.}\label{fig:reset1}
    \end{subfigure}
    \hspace*{\fill}   % maximize separation between the subfigures
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.475\textwidth}
        \includegraphics[width=\textwidth]{img/reset2_labeled.png}
        \caption{Turning to face the best resetting direction. The physical user turns a little more than $180^\circ$ to their right, while the virtual user turns $360^\circ$ to the right.}\label{fig:reset2}
    \end{subfigure}
    \caption{A visualization of the two steps involved in resetting: \autoref{fig:reset1} Shows selecting the best direction for resetting. \autoref{fig:reset2} Shows the user to turning to face the best direction.}\label{fig:reset}
\end{figure}

% === outline ===
% - define alignment
% - describe what it means for a controller to use alignment
% - explain the state descriptor we use to guide the alignment process (position/orientation/vis poly)
% sections:
%     - basic/general definition
%     - state description + comparison metrics
%     - alignment maneuvers (IF I CAN IMPLEMENT THIS IN TIME)
%     - advantages and disadvantages of alignment heuristic

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> notes.tex <==
- We used Reset to gradient to allow for easier comparison. Reset to center works only for empty environments (Bachmann et al), but our environments are sometimes not empty (environments from Thomas et al). Furthermore, the baseline no redirection condition uses reset to center (Azmandian et al 2015), so we need to use a no redirection method if we want to test the efficacy of their "relative effectiveness" metric. But the Azmandian paper also uses an empty physical space, so reset to center works for them, but it doesn't work for us. Basically the same as the Bachmann paper: We need to use reset-to-gradient to make all the conditions easily comparable.
    - We note that this relatively minor problem in itself highlights the difficulty of comparing different RDW controllers, which is just more evidence for the purpose of this paper.

==> results.tex <==
\section{Results} \label{results}
We performed quantitative evaluations of the performance of S2C, APF, and ARC using four metrics (\autoref{subsec:evaluation}).
Each of the metrics was computed for all 50 paths in each condition.
RDW algorithms can sometimes occasionally encounter ``unlucky'' virtual paths that make it particularly difficult to avoid collisions.
To make our comparisons robust to these unlucky paths, outliers in the data that were $1.5$ times larger than the interquartile range of the data were replaced with the median of the data.
We evaluated the normality of the data using visual inspection of Q-Q plots and histograms as well as measures of the distributions' skew and kurtosis.
Homoscedasticity was evaluated using Levene's test.
For each metric measured, the assumption of normality or homoscedasticity was violated, so we conducted all of our tests using a robust one-way repeated measures $20\%$ trimmed means ANOVA (using the WRS2 package).
Pairwise post-hoc comparisons were computed using linear contrasts.

Due to the large sample size in our experiments, we report $95\%$ confidence interval instead of \textit{p}-values.
As the sample size grows, statistical tests become sensitive to even minute differences between samples, and the \textit{p}-value becomes unreliable as it approaches $0$.
Furthermore, reporting confidence intervals allows for easier comparisons with future work if they also report confidence intervals, since the interval provides numerical bounds on the differences between conditions \cite{lin2013research}.

% - we replaced outliers with the median value to make comparisons more robust (rdw can be succeptible to outliers)
% - normality was tested using qq plots, histograms, and measure of skewness and kurtosis. large sample size makes the norm test unreliable (shapiro wilks? don't remember the name)
% - we report confidence intervals because large sample size (only 100 paths, but each path has a lot of data). also, CIs is better for comparing against other research if they also report CIs. \cite{lin2013research}
% - i shoudl report my p values as p<0.001 when R tells me they are p=0
% - the degrees of freedom in the ANOVA are not integers because sphericity is violated, and the function automatically does a correctoion to account for this, which makes the DoF smaller than normal

\subsection{Experiment 1}
\label{results:exp1}
Experiment 1 was conducted in Environment A.
\subsubsection{Number of resets}
The number of collisions for each steering controller is shown in \autoref{fig:envA_resets}.
We found a significant effect of steering controller on the number of resets $F(1.87,54.1)=62.7981, p<.0001$.
Post-hoc tests showed a significant difference between S2C and ARC $(\hat{\psi}=11.0 \ [8.62, 13.4])$.
This can be interpreted as meaning that for $95\%$ of paths, S2C will incur $8.62$ to $13.4$ more collisions than ARC will.
We also found a significant difference between APF and ARC $(\hat{\psi}=4.77 \ [2.21, 7.32])$.
So, APF will encounter 2.21 to 7.32 more collisions than ARC will on $95\%$ of paths.
Finally, there was a significant difference between S2C and APF $(\hat{\psi}=5.73 \ [3.85, 7.61])$.
On $95\%$ of trials, S2C had 3.85 to 7.61 more collisions than APF.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envA_resets.png}
    \caption{The number of resets for each redirection controller in Environment A. The boxplots show the median and IQR for the data. A significant difference was found between all algorithms, with ARC outperforming both S2C and APF.}
    \label{fig:envA_resets}
\end{figure}
% - failed levene's test: 
%       Df F value  Pr(>F)  
% group   2  4.2957 0.01538 *
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 62.7981 
% Degrees of freedom 1: 1.87 
% Degrees of freedom 2: 54.1 
% p-value: 0
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad    5.73333  3.85357  7.61309   0e+00 0.0250 TRUE
% S2C vs. Align     11.00000  8.61974 13.38026   0e+00 0.0169 TRUE
% APFGrad vs. Align  4.76667  2.21251  7.32082   5e-05 0.0500 TRUE

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A boxplot of the average distance walked between resets for each controller is shown in \autoref{fig:envA_distance}.
There was a significant effect of controller on the distance walked $F(1.04,30.13)=19.0171, p<.0001$.
We found a significant difference between S2C and ARC $(\hat{\psi}=-21.3 \ [-31.8, -10.8])$.
On $95\%$ of paths, ARC allowed the user to walk 10.8 to 31.8 meters further than S2C did.
There was also a significant difference between APF and ARC $(\hat{\psi}=-15.3 \ [-24.4, -6.24])$.
The user was able to walk 6.24 to 24.4 meters further with ARC than with APF on $95\%$ of trials.
The post-hoc test also revealed a significant difference between S2C and APF $(\hat{\psi}=-4.80 \ [-6.61, -3.00])$.
Thus, APF allowed users to travel 3.00 to 6.61 meters further than S2C did on $95\%$ of trials.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envA_distance.png}
    \caption{The average distance walked between resets for each path with each controller in Environment A. Significant differences were found between all controllers. On average, ARC allowed the user to walk further before being reset due to a collision. The average distance for some paths is quite high because ARC was able to achieve alignment and steer the user along a collision-free path.}
    \label{fig:envA_distance}
\end{figure}
% - failed levene's test:
%       Df F value    Pr(>F)    
% group   2  22.716 2.531e-09 ***
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 19.0171 
% Degrees of freedom 1: 1.04 
% Degrees of freedom 2: 30.13 
% p-value: 0.00012
%                      psihat  ci.lower  ci.upper p.value p.crit  sig
% S2C vs. APFGrad    -4.80450  -6.61015  -2.99885 0.00000 0.0169 TRUE
% S2C vs. Align     -21.29273 -31.81897 -10.76649 0.00002 0.0250 TRUE
% APFGrad vs. Align -15.32331 -24.40404  -6.24257 0.00018 0.0500 TRUE

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The distribution of average distance walked between resets across all trials is shown in \autoref{fig:envA_alignment}.
The robust trimmed means ANOVA revealed a significant effect of steering controller on the user's average alignment $F(1.55,44.88)=4248.276,p<.0001$.
After conducting post-hoc comparisons, we found a significant difference between S2C and ARC $(\hat{\psi}=1.33 \ [1.29, 1.37])$.
Navigation with ARC was able to keep the user's alignment 1.29 to 1.37 lower than with S2C for $95\%$ of trials.
There was a significant difference between APF and ARC $(\hat{\psi}=1.20 \ [1.17, 1.23])$, meaning that ARC maintained an alignment that was 1.17 to 1.23 lower than the average alignment achieved using APF.
Finally, there was a significant difference between S2C and APF $(\hat{\psi}=0.131 \ [0.102, 0.160])$, meaning that users were 0.102 to 0.160 more aligned when walking with APF than with S2C.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envA_alignment.png}
    \caption{The average alignment for the user in Environment A when steered with each controller. As expected, ARC maintained a low alignment score, while S2C and APF did not. Alignment measures the difference between the user's physical and virtual states, so a lower alignment is better.}
    \label{fig:envA_alignment}
\end{figure}
% - Failed levene's test:
%       Df F value    Pr(>F)    
% group   2  17.193 1.953e-07 ***
%       147
% - not normally distirbuted
% - run robust trimmed means anova
% Test statistic: F = 4248.276 
% Degrees of freedom 1: 1.55 
% Degrees of freedom 2: 44.88 
% p-value: 0 
%                   psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   0.13131  0.10252  0.16011       0 0.0500 TRUE
% S2C vs. Align     1.33481  1.29061  1.37901       0 0.0250 TRUE
% APFGrad vs. Align 1.20026  1.16676  1.23376       0 0.0169 TRUE

% \subsubsection{Steering rate}
% % $(\hat{\psi}=xxx \ [xxx, xx])$
% The average curvature gain applied while the user walked, across all paths, is shown in \autoref{fig:envA_steering}.
% There was a significant effect of controller on the steering rate $F(1.02,29.63)=171.0561,p<.0001$.
% Post-hoc tests showed a significant difference between S2C and ARC $(\hat{\psi}=1.98 \ [1.43, 2.53])$, indicating that the user experienced $1.42^\circ$ to $2.53^\circ$ more redirection per second on $95\%$ of trials with S2C than with ARC.
% There was also a significant difference between APF and ARC $(\hat{\psi}=3.12 \ [2.59, 3.63])$.
% Users experienced $2.59^\circ$ to $3.63^\circ$ more redirection per second when locomoting with APF than with ARC.
% We also found a significant difference in steering rate between S2C and APF $(\hat{\psi}=-1.13 \ [-1.19, -1.06])$, meaning that users were redirected $1.06^\circ$ to $1.19^\circ$ more per second with APF than with S2C on $95\%$ of paths.
% - failed levene's test:
%       Df F value    Pr(>F)    
% group   2   91.32 < 2.2e-16 ***
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 171.0561 
% Degrees of freedom 1: 1.02 
% Degrees of freedom 2: 29.63 
% p-value: 0 
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   -1.12704 -1.18938 -1.06471       0 0.0169 TRUE
% S2C vs. Align      1.97651  1.42568  2.52734       0 0.0500 TRUE
% APFGrad vs. Align  3.10942  2.59151  3.62732       0 0.0250 TRUE

\subsubsection{Amount of time redirected}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The percentage of frames that redirection was applied across all paths is shown in \autoref{fig:envA_amount_redir}.
We found a significant effect of controller on the percentage of frames for which redirection was applied $F(1.01,29.2)=20.1351,p<.0001$.
There was a significant difference between S2C and ARC $(\hat{\psi}=0.000362 \ [0.000168, 0.00556])$, indicating that the user was redirected for $00168\%$ to $0.556\%$ more frames with S2C than with ARC on $95\%$ of paths.
Additionally, there was a significant difference between APF and ARC $(\hat{\psi}=0.00328 \ [0.00131, 0.00525])$.
That is, APF redirected the user on $0.131\%$ to $0.525\%$ more frames than ARC did, on $95\%$ of paths.
Finally, we found a significant difference difference between S2C and APF $(\hat{\psi}=0.031 \ [0.020, 0.041])$, which means that on $95\%$ of trials, the user was redirected for $0.020\%$ to $0.041\%$ more frames when being redirected with S2C than with APF.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envA_amount_redir.png}
    \caption{Percentage of frames for which redirection gains were applied across all paths, for each controller in Environment A. S2C and APF had a similar amount of frames spent redirecting (more than $99\%$), while on some paths ARC was able to redirect the user for less tan $96\%$ of frames.}
    \label{fig:envA_amount_redir}
\end{figure}
% - failed levene's test
%       Df F value    Pr(>F)    
% group   2  18.281 8.123e-08 ***
%       147 
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 20.1351 
% Degrees of freedom 1: 1.01 
% Degrees of freedom 2: 29.2 
% p-value: 1e-04 
%                   psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   0.00031  0.00020  0.00041 0.00000 0.0169 TRUE
% S2C vs. Align     0.00362  0.00168  0.00556 0.00005 0.0250 TRUE
% APFGrad vs. Align 0.00328  0.00131  0.00525 0.00022 0.0500 TRUE

\subsubsection{Qualitative Evaluations}
The heat map of the physical space for Environment A is shown in \autoref{fig:envA_combined_heatmap}.
Every controller had the user spend most of their time near the center of the environment.
This is what S2C is designed to do, and APF reduces to S2C in empty environments, so this is no surprise.
One interesting thing to note, however, is that the user spends less time at the center of the room compared to S2C and APF.

\autoref{fig:resets_by_CR} shows that in Environment A, S2C is outperformed by APF and ARC, and APF is outperformed by ARC.
The difference in performance between ARC and APF is larger than the performance difference of APF and S2C.
This is because ARC is able to steer the user on collision-free paths if the physical and virtual states are close enough that ARC can cause the system to become perfectly aligned.
Once this happens, redirection is no longer needed since the PE and VE are identical.
This never happens with S2C or APF.

The frequency plot of curvature gains applied by each controller is shown in \autoref{fig:envA_steering}.
The implementation of APF we used \cite{thomas2019general} always applies maximum curvature gain.
However, S2C and ARC do not always apply the maximum curvature gain.
The average curvature gain for each path steered by S2C is always above $6^\circ$, which is still fairly high considering the perceptual limit is about $7.6^\circ$.
On the other hand, ARC is able to apply curvature gains much lower than the perceptual limit and with high consistency.
All of the average gains applied by ARC are below $7^\circ$, and they are nicely distributed across the whole range of possible gains.
This shows that ARC applies less intense gains much more often than other controllers, which creates a more comfortable experience for the user.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envA_combined_heatmap.pdf}
    \caption{A heat map of the user's physical position across all paths for each controller in Environment A. Yellow tiles indicate the most time spent at that location, while purple tiles indicate the least amount of time. S2C and APF steer the user such that they spent the large majority of their time in the center of the room, while ARC allows the user to visit each region of the room more evenly.}
    \label{fig:envA_combined_heatmap}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envA_steering.png}
    \caption{A histogram of the average curvature gain applied by each controller for each path in Environment A. The implementation of APF we used always applies the same gain, while S2C and ARC apply lower gains on average. S2C still applies gains fairly close to the perceptual threshold ($\approx 7.6^\circ /s$), but ARC is able to steer the user on paths with fewer collisions and significantly reduced curvature gains. Most of the gains applied by ARC fall in the $3^\circ/s - 5^\circ /s$ range, showing that ARC only applies the gains necessary to avoid collisions and maintain alignment.}
    \label{fig:envA_steering}
\end{figure}

\subsection{Experiment 2}
Experiment 2 was conducted in Environment B.
\subsubsection{Number of resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The boxplot showing the distribution of number of resets across all paths for each steering controller is shown in \autoref{fig:envB_resets}.
The robust ANOVA revealed a significant effect of controller on the number of resets $F(1.33,38.68)=38.7793,p<.0001$.
The pairwise post-hoc comparisons revealed a significant difference between S2C and ARC $(\hat{\psi}=41.7 \ [28.4, 55.0])$.
Therefore, on $95\%$ of trials, the user experienced 28.4 to 55.0 more collisions when navigating using S2C than with ARC.
We also found a significant difference in number of resets between APF and ARC $(\hat{\psi}=7.65 \ [1.52, 13.8])$, which means that on $95\%$ of trials, the user collided with an obstacle 1.53 to 13.8 more times using APF than when using ARC.
Lastly, we saw a significant difference between S2C and APF $(\hat{\psi}=31.9 \ [16.9, 47.0])$, showing that the user incurred 16.9 to 47.0 more collisions when being steered with S2C than when being steered with APF, on $95\%$ of paths.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envB_resets.png}
    \caption{The number of resets across all paths for each redirection controller in Environment B. ARC and APF have somewhat similar performance, but ARC still achieves a lower spread and median number of resets than APF. S2C performs much worse than ARC and APF due to the obstacles placed in the physical room (see \autoref{fig:environments}).}
    \label{fig:envB_resets}
\end{figure}
% - failed levene's test:
% group   2  20.985 9.615e-09 ***
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 38.7793 
% Degrees of freedom 1: 1.33 
% Degrees of freedom 2: 38.68 
% p-value: 0
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   31.91667 16.88978 46.94356 0.00001 0.0250 TRUE
% S2C vs. Align     41.70000 28.43561 54.96439 0.00000 0.0169 TRUE
% APFGrad vs. Align  7.65000  1.52062 13.77938 0.00357 0.0500 TRUE

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A plot of the average distances walked between resets for all paths with all controllers is shown in \autoref{fig:envB_distance}.
There was a significant effect of steering algorithm on the average distance walked between resets $F(1.89,54.76)=53.8905,p<.0001$.
After conducting post-hoc pairwise comparisons, we found a significant difference between S2C and ARC $(\hat{\psi}=-0.906 \ [-1.12, -0.703])$, which shows that on $95\%$ of paths, when the user navigates with ARC, they traveled an average of 0.703 to 1.12 meters more than if they navigated with S2C.
A significant difference between APF and ARC $(\hat{\psi}=-0.274 \ [-0.487, -0.061])$ indicated that the user was able to travel 0.061 to 0.487 meters further using ARC than they were able to when using APF for redirection.
Finally, a significant difference between S2C and APF $(\hat{\psi}=-0.635 \ [-0.868, -0.402])$ showed that the simulated user was able to walk 0.402 to 0.868 meters further with APF than with S2C as the redirection controller.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envB_distance.png}
    \caption{The average physical distance walked between resets across all paths for each controller in Environment B. We see a similar pattern to the number of resets, wherein ARC and APF have similar performances with ARC achieving a higher distance walked, and S2C performs poorly and often requires resets after walking less than $1m$, as indicated by the long whiskers of the purple boxplot.}
    \label{fig:envB_distance}
\end{figure}
% - failed levene's test:
%       Df F value  Pr(>F)  
% group   2  4.6503 0.01101 *
%       147
% - was normally distributed
% - ran robust trimmed means anova
% Test statistic: F = 53.8905 
% Degrees of freedom 1: 1.89 
% Degrees of freedom 2: 54.76 
% p-value: 0 
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   -0.63488 -0.86764 -0.40211 0.00000 0.0250 TRUE
% S2C vs. Align     -0.90571 -1.10827 -0.70315 0.00000 0.0169 TRUE
% APFGrad vs. Align -0.27398 -0.48717 -0.06079 0.00281 0.0500 TRUE

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The average alignment scores for all controllers in Environment B are shown in \autoref{fig:envB_alignment}.
A significant effect of redirection controller on the user's average alignment was found $F(1.27,36.81)=194.2711,p<.0001$.
Using pairwise post-hoc tests, we determined which algorithms outperformed which.
There was a significant difference between S2C and ARC $(\hat{\psi}=0.328 \ [0.256, 0.400])$, which means that on $95\%$ of paths, the user had 0.256 to 0.400 more alignment score when using S2C than when using ARC.
We also found a significant difference between APF and ARC $(\hat{\psi}=0.492 \ [0.464, 0.519])$.
Therefore, the user's alignment score was 0.464 to 0.519 higher when steered with APF than when steered with ARC.
Finally, there was a significant difference between S2C and APF $(\hat{\psi}=-0.162 \ [-0.237, -0.089])$, which tells us that on $95\%$ of paths walked, the user's alignment score was 0.089 to 0.237 higher when walking with APF than with S2C.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envB_alignment.png}
    \caption{Average alignment score of the user over all paths in Environment B, for all redirection controllers. ARC is able to maintain a relatively low alignment score (a score of 0 indicates perfect alignment), while S2C and APF exhibit higher alignment scores. This is not unexpected since APF and S2C are not designed using alignment, but it indicates that ARC is working as intended.}
    \label{fig:envB_alignment}
\end{figure}
% - failed levene's test:
%       Df F value    Pr(>F)    
% group   2  44.624 7.166e-16 ***
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 194.2711 
% Degrees of freedom 1: 1.27 
% Degrees of freedom 2: 36.81 
% p-value: 0 
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   -0.16246 -0.23664 -0.08829   1e-05 0.0500 TRUE
% S2C vs. Align      0.32788  0.25550  0.40026   0e+00 0.0250 TRUE
% APFGrad vs. Align  0.49173  0.46406  0.51940   0e+00 0.0169 TRUE

% \subsubsection{Steering rate}
% % $(\hat{\psi}=xxx \ [xxx, xx])$
% The distribution of average curvature gains applied by each steering algorithm across all 50 paths in Environment B is shown in \autoref{fig:envB_steering}.
% The robust ANOVA revealed a significant effect of controller on the steering rate $F(1.07,31.13)=3000.03,p<.0001$.
% Pairwise comparisons showed that ARC steered the user significantly less than S2C $(\hat{\psi}=-0.314 \ [-0.448, -0.179])$, indicating that the user was steered $0.448^\circ$ to $0.179^\circ$ less while walking with ARC than with S2C.
% There was also a significant difference between APF and ARC $(\hat{\psi}=2.48 \ [2.36, 2.60])$, showing that on $95\%$ of paths, the user was steered $2.36^\circ$ to $2.60^\circ$ less with ARC than APF when walking.
% Lastly, there was a significant difference between S2C and APF $(\hat{\psi}=-2.80 \ [-2.83, -2.77])$, which tells us that on $95\%$ of trials, the user experienced $2.83^\circ$ to $2.77^\circ$ less redirection per second while walking with S2C than with APF.
% - failed levene's test:
%       Df F value    Pr(>F)    
% group   2  56.113 < 2.2e-16 ***
%       147  
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 3000.03 
% Degrees of freedom 1: 1.07 
% Degrees of freedom 2: 31.13 
% p-value: 0
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   -2.79969 -2.82572 -2.77366       0 0.0250 TRUE
% S2C vs. Align     -0.31350 -0.44820 -0.17881       0 0.0500 TRUE
% APFGrad vs. Align  2.48037  2.36121  2.59952       0 0.0169 TRUE

\subsubsection{Amount of time redirected}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The distribution of percentage of frames redirected per path for all controllers is shown in \autoref{fig:envB_percent}.
We found a significant effect of controller on the percentage of frames for which redirection was applied $F(1.88,54.59)=73.9954,p<.0001$.
By conducting post-hoc tests, we found a significant difference between S2C and ARC $(\hat{\psi}=0.00104 \ [0.00076, 0.00131])$, which means that for $95\%$ of paths, the user was redirected $0.076\%$ to $0.131\%$ less with ARC than with S2C.
We also saw a significant difference between APF and ARC $(\hat{\psi}=0.00056 \ [0.00034, 0.00078])$.
The simulated user was redirected $0.034\%$ to $0.078\%$ less with ARC than with APF on $95\%$ of trials.
We also saw a significant difference between S2C and APF $(\hat{\psi}=0.00046 \ [0.00030, 0.00062])$, indicating that the user was redirected $0.046\%$ to $0.030\%$ less with APF than with S2C.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envB_percent.png}
    \caption{The percentage of frames for which redirection was applied, for each controller in Environment B. Environment B is fairly complex ($CR = 0.861$), so all controllers, including ARC, must constantly apply redirection to avoid collisions.}
    \label{fig:envB_percent}
\end{figure}
% - did not fail levene's test:
%       Df F value Pr(>F)
% group   2  0.2165 0.8056
%       147
% - was not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 73.9954 
% Degrees of freedom 1: 1.88 
% Degrees of freedom 2: 54.49 
% p-value: 0
%                   psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   0.00046  0.00030  0.00062       0 0.0250 TRUE
% S2C vs. Align     0.00104  0.00076  0.00131       0 0.0169 TRUE
% APFGrad vs. Align 0.00056  0.00034  0.00078       0 0.0500 TRUE

\subsubsection{Qualitative Evaluations}
The heat map showing the user's occupancy in the physical space for Environment B is shown in \autoref{fig:envB_combined_heatmap}.
S2C and APF have very similar heat maps since both algorithms steer the user towards the center of the space.
APF steers the user towards the center because it is the most open space in the environment, furthest away from all obstacles.
The heat map for ARC shows that the user is steered all around the physical room.
Interestingly, there is some bias in that the user tends to be along the top wall of the room.
The reason for this is not clear, and further work should be done to better understand biases like this.

The number of resets for each algorithm in Environment B are compared in \autoref{fig:resets_by_CR}.
As expected, the number of resets increases for all controllers, since Environment B is more complex than Environment A.
Interestingly, however, the difference in performance between ARC and the other algorithms is much smaller than it was in Environment A.
This is likely related to ARC's tendency to steer the user near the top wall, but it is possible that there is another reason for ARC's relatively worse performance versus its performance in Environment A.

\autoref{fig:envB_steering} shows the average curvature gain applied by each controller over all paths in Environment B.
Much like Environment A, S2C and ARC apply weaker gains than APF.
One difference between Environment A and B is that ARC applies stronger gains more often than S2C.
The spread of gains applied by ARC is also much smaller than it was in Environment A, which is likely because ARC was not able to achieve perfect alignment and thus was not able to apply weak gains while also lowering the user's alignment score.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envB_combined_heatmap.pdf}
    \caption{A heat map of the physical locations visited by the user in Environment B when steered with each controller. Yellow tiles indicate more visits to a region, while purple tiles indicate less time spent in a region. Obstacles are shown in black. S2C and APF keep the user concentrated near the center of the room since it is the most open space in all directions, while ARC is able to utilize more of the space and steer the user along all corridors in the room. ARC has some tendency to keep the user near the north wall of the room, which we suspect is due to the user getting stuck in between obstacles, but the exact cause is not clear.}
    \label{fig:envB_combined_heatmap}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envB_steering.png}
    \caption{A histogram of the average curvature gain applied for each path with each controller in Environment B. As in Environment A, APF applies a constant curvature gain when the user is walking. S2C and ARC apply gains with an average in the range of $4^\circ/s - 6^\circ/s$, with ARC applying gains all gains at a lower intensity than about half of the gains applied by S2C. Note that the lowest gains applied by S2C are lower than those of ARC.}
    \label{fig:envB_steering}
\end{figure}

\subsection{Experiment 3}
Experiment 3 was conduct in Environment C.
\subsubsection{Number of resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A boxplot of the number of collisions incurred in Environment C with all controllers on each path is shown in \autoref{fig:envC_resets}
There was a significant effect of controller on the number of resets $F(1.04,30.05)=676.688,p<.0001$.
Post-hoc pairwise comparisons revealed a significant difference between S2C and ARC $(\hat{\psi}=993.4 \ [901.555, 1085.245])$.
This means the user collided with physical obstacles 901.555 to 1085.45 times more when steered by S2C than they did when steered by ARC, on $95\%$ of trials.
We also found a significant difference between APF and ARC $(\hat{\psi}=75.0 \ [60.414, 89.586])$, which indicates that the user incurred 60.414 to 89.586 less collisions when steered by ARC than when steered by APF.
Finally, there was a significant difference between S2C and APF $(\hat{\psi}=919.8 \ [829.53, 1010.069])$, showing that the user had 829.53 to 1010.069 more collisions on $95\%$ of paths when steered with S2C than when steered with APF.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envC_resets.png}
    \caption{The number of resets on each path for each controller in Environment C. Again, S2C has a very poor performance, but this time it is due to the obstacle occupying the center of the room. ARC has a lower reset rate than APF, and also has a much lower variance in numbers of resets, indicating that in highly complex environments like Environment C ($CR = 0.562$), the user can be consistently steering with a relatively low number of resets.}
    \label{fig:envC_resets}
\end{figure}
% - failed levene's test
% group   2  70.181 < 2.2e-16 ***
%       147  
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 676.688 
% Degrees of freedom 1: 1.04 
% Degrees of freedom 2: 30.05 
% p-value: 0 
%                   psihat  ci.lower   ci.upper p.value p.crit  sig
% S2C vs. APFGrad    919.8 829.53040 1010.06960       0 0.0250 TRUE
% S2C vs. Align      993.4 901.55471 1085.24529       0 0.0169 TRUE
% APFGrad vs. Align   75.0  60.41413   89.58587       0 0.0500 TRUE

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The distributions of average distances walked between resets for all controllers in Environment C is shown in \autoref{fig:envC_distance}.
A robust ANOVA indicated a significant effect of controller on the average physical distance walked by the user between resets $F(1.51,43.67)=1635.269,p<.0001$.
Post-hoc tests showed a significant difference between S2C and ARC $(\hat{\psi}=-3.799 \ [-3.912, -3.687])$, which tells us that on $95\%$ of paths, the user was able to walk 3.687 to 3.912 meters further when steered with ARC than with S2C.
We also saw a significant difference between APF and ARC $(\hat{\psi}=-2.443 \ [-2.632, -2.256])$.
That is, the user was able to walk 2.256 to 2.632 meters further when using ARC than when using APF, on $95\%$ of paths.
There was also a significant difference between S2C and APF $(\hat{\psi}=-1.346 \ [-1.519, -1.172])$, showing that the user walked 1.172 to 1.519 meters further when using APF than when using S2C.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envC_distance.png}
    \caption{Average distance walked between resets on each path for all controllers in Environment C. S2C has a poor performance due to being constantly reset and redirected back to the obstacle in the center of the room. APF allows the user to walk further than S2C does, but still often triggers a reset less than every $2m$. The long upper whisker on the APF boxplot indicates that APF can achieve decent performance on some paths. ARC is able to steer the user much further than APF on all paths, with a median distance walked between resets of $4m$.}
    \label{fig:envC_distance}
\end{figure}
% - failed levene's test:
% group   2  32.014 2.876e-12 ***
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 1636.269 
% Degrees of freedom 1: 1.51 
% Degrees of freedom 2: 43.67 
% p-value: 0 
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   -1.34567 -1.51927 -1.17207       0 0.0500 TRUE
% S2C vs. Align     -3.79924 -3.91161 -3.68686       0 0.0250 TRUE
% APFGrad vs. Align -2.44376 -2.63188 -2.25564       0 0.0169 TRUE

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A plot of the average alignment score across 50 paths for all controllers is shown in \autoref{fig:envC_alignment}.
We found a significant effect of steering controller on the user's average alignment $F(1.92,55.69)=1363.52,p<.0001$.
After doing pairwise comparisons to find the exact difference between controllers, we found a significant difference between S2C and ARC $(\hat{\psi}=-0.980 \ [-1.04, -0.921])$, which tells us that the user's alignment score was 0.921 to 1.04 higher when being redirected with ARC than with S2C.
Additionally, there was a significant difference between APF and ARC $(\hat{\psi}=0.174 \ [0.121, 0.226])$.
The simulated user's alignment score was 0.121 to 0.226 lower when using ARC than when using APF.
Lastly, there was a significant difference between S2C and APF $(\hat{\psi}=-1.129 \ [-1.189, -1.069])$.
The user's alignment score was 1.069 to 1.189 lower when walking with S2C than with APF.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envC_alignment.png}
    \caption{The average alignment score for all paths with each controller in Environment C. Interestingly, S2C achieves the best (lowest) alignment score, despite have a very high number of resets and low travel distance between resets. ARC achieves an alignment score lower than APF, but worse than S2C. The reason for this is not clear, since S2C is not designed around alignment. This suggests that measuring alignment score may not be the most useful metric, since ARC is able to achieve much better performance than S2C, but still has a worse alignment score.}
    \label{fig:envC_alignment}
\end{figure}
% - did not fail levene's test:
%       Df F value Pr(>F)
% group   2  1.1752 0.3116
%       147
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 1363.52 
% Degrees of freedom 1: 1.92 
% Degrees of freedom 2: 55.69 
% p-value: 0 
% S2C vs. APFGrad   -1.12905 -1.18946 -1.06865       0 0.0250 TRUE
% S2C vs. Align     -0.97955 -1.03774 -0.92137       0 0.0169 TRUE
% APFGrad vs. Align  0.17357  0.12074  0.22640       0 0.0500 TRUE

% \subsubsection{Steering rate}
% % $(\hat{\psi}=xxx \ [xxx, xx])$
% There was a significant effect of redirection controller on the steering rate $F(1.41,40.96)=690.5261,p<.0001$.
% Using post-hoc tests, we found a significant difference between S2C and ARC $(\hat{\psi}=0.104 \ [-0.006, 0.213])$, telling us that the user was steered 
% - failed levene's test:
% group   2  44.697 6.848e-16 ***
%       147  
% - not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 690.5261 
% Degrees of freedom 1: 1.41 
% Degrees of freedom 2: 40.96 
% p-value: 0 
%                     psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   -1.09342 -1.15282 -1.03402  0.0000 0.0250 TRUE
% S2C vs. Align      0.10353 -0.00613  0.21319  0.0231 0.0500 TRUE
% APFGrad vs. Align  1.19306  1.10435  1.28177  0.0000 0.0169 TRUE

\subsubsection{Amount of time redirected}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A plot of the amount of frames where redirection was applied across all paths for all controllers is shown in \autoref{fig:envC_percentage}.
There was a significant effect of controller on the percentage of frames where redirection was applied $F(2,58)=731.0069,p<.0001$.
Post-hoc tests showed a significant difference between S2C and ARC $(\hat{\psi}=0.00272 \ [0.00254, 0.00290])$, meaning that the user was redirected $0.245\%$ to $0.290\%$ less with ARC than with S2C.
We also found a significant difference between APF and ARC $(\hat{\psi}=0.00133 \ [0.00115, 0.00150])$.
The simulated user was redirected on $0.115\%$ to $0.150\%$ fewer frames with ARC than with APF.
Finally, there was a significant difference between S2C and APF $(\hat{\psi}=0.00137 \ [0.00118, 0.00155])$, indicating that the user was steering with redirection $0.118\%$ to $0.155\%$ less with S2C than with APF.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envC_percentage.png}
    \caption{Percentage of frames for which redirection was applied, for each redirection controller in Environment C. Since Environment C is very complex, with multiple obstacles in the physical and virtual environments, the user has to be steered almost always, regardless of the controller being used.}
    \label{fig:envC_percentage}
\end{figure}
% - failed levene's test:
%       Df F value    Pr(>F)    
% group   2  33.679 9.102e-13 ***
%       147  
% - was not normally distributed
% - run robust trimmed means anova
% Test statistic: F = 731.0069 
% Degrees of freedom 1: 2 
% Degrees of freedom 2: 58 
% p-value: 0
%                   psihat ci.lower ci.upper p.value p.crit  sig
% S2C vs. APFGrad   0.00137  0.00118  0.00155       0 0.0500 TRUE
% S2C vs. Align     0.00272  0.00254  0.00290       0 0.0250 TRUE
% APFGrad vs. Align 0.00133  0.00115  0.00150       0 0.0169 TRUE

\subsubsection{Qualitative Evaluations}
A heat map of the user in the physical space for Environment C is shown in \autoref{fig:teaser}.
The black rectangles represent obstacles in the environment, and purple tiles indicate low frequency of the user being in that area, while yellow tiles indicate high frequency.
It is clear that ARC utilizes the PE to its fullest potential, evidenced by the relatively uniform green color across the whole free space.
APF does worse than ARC at using all of the space available in the PE, with the user being concentrated mostly in the open space in the bottom corner of the room.
The user is able to walk through the other regions in the room sometimes, but the algorithm shows a clear bias towards the largest free space in the room.
S2C performs very poorly, since there is an obstacle in the center of the physical room.
The user is constantly redirected towards the center, only to be turned away when they get too close, and then steered right back to the center.
The high concentration near the center of the room is supported by the very high number of resets they incurred in this space (see \autoref{fig:envC_resets}).

The performance of ARC, APF, and S2C is also compared in \autoref{fig:resets_by_CR}.
ARC achieves much fewer resets than either APF or S2C in Environment C, which is the most complex, which highlights ARC's ability to handle physical and virtual environments with differing configurations and complexities.

Finally, \autoref{fig:envC_steering} shows a frequency plot of the gains applied by each controller across all paths in Environment C.
As expected, APF applies the maximum curvature gain for each frame.
However, all gains applied by both ARC and S2C are lower than that of APF, with ARC applying the lowest gains of all, and applying stronger gains less often than S2C.
This shows a major strength of our algorithm: ARC is able to achieve a lower number of resets than current state of the art while also applying \textit{less intense} gains.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/resets_by_CR.png}
    \caption{The relationship between the environment complexity and the number of resets incurred by a redirection controller. ARC consistently has a better performance than S2C and APF for all environment complexities. The performance difference between ARC and the other algorithms is quite large for environments A and C, but the difference decreases drastically for Environment B. It is not clear why Environment B causes the controllers to have a more similar performance, but it may be due to the relatively few pathing options afforded by the narrow hallways of Environment B. Environments A and C both include regions with a fairly large amount of open space, unlike Environment B (see \autoref{fig:environments}).}
    \label{fig:resets_by_CR}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/Old small data/envC_steering.png}
    \caption{The average curvature gain applied by each controller for all paths in Environment C. The same trend as in Environment B is seen here, where APF has a higher steering rate than S2C and ARC. One difference between the steering rates in Environment B and C is that the gains applied by S2C and ARC are in a higher range ($6^\circ/s - 7^\circ/s$) in Environment C than they were in Environment B ($4^\circ/s - 6^\circ/s$).}
    \label{fig:envC_steering}
\end{figure}


==> results2.tex <==
\section{Results} \label{results}
We performed quantitative evaluations of the performance of S2C, APF, and ARC using three quantitative metrics and three qualitative (\autoref{subsec:evaluation}).
Each of the metrics was computed for all 100 paths in each condition.
In complex environments, RDW controller algorithms can sometimes encounter ``unlucky'' virtual paths that make it particularly difficult to avoid collisions, and the user will end up incurring many collisions in a small time frame (they essentially get ``stuck'' on an obstacle).
To make our comparisons robust to these unlucky paths, outliers in the data that were $1.5$ times larger than the interquartile range of the data were replaced with the median of the data.
We evaluated the normality of the data using visual inspection of Q-Q plots and histograms as well as measures of the distributions' skew and kurtosis.
Homoscedasticity was evaluated using Levene's test.
For each metric measured, the assumption of normality or homoscedasticity was violated, so we conducted all of our tests using a robust one-way repeated measures $20\%$ trimmed means ANOVA (using the WRS2 package).
Pairwise post-hoc comparisons were computed using linear contrasts.

Due to the large sample size in our experiments, we report $95\%$ confidence interval instead of \textit{p}-values.
As the sample size grows, statistical tests become sensitive to small and minute differences between samples, and the \textit{p}-value becomes unreliable as it approaches $0$.
Confidence intervals, however, become narrower as the sample size grows, meaning they are able to scale with the sample size and are still reliable for experiments with large samples.
Furthermore, reporting confidence intervals allows for easier comparisons with future work if they also report confidence intervals, since the interval provides numerical bounds on the differences between conditions \cite{lin2013research}.

The results are shown in \autoref{tab:results}, with discussions in subsequent sections.
Most of the discussion is limited to comparing ARC to APF, since it is already well-established that APF outperforms S2C \cite{thomas2019general, bachmann2019multi}.
A confidence interval that does not contain 0 in its range [CI lower, CI upper] is considered to be significant.
Thus, we found significant differences between all groups in our post-hoc tests.
The common pattern seen in the results is that ARC outperforms APF and S2C, while APF outperforms S2C.
One condition for which this was not the case is the alignment metric in Environment C.
% Full descriptive statistics for each metric for each controller are in the supplemental materials \autoref{}.

\textbf{[need to mention that the alignment comparison between APF and S2C doesn't make sense since neiter algortihm considers alignment. maybe put it in the metrics section of section 4?]}

\begin{table*}[ht]
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
    \multicolumn{10}{c}{\textbf{Environment A}}    \\ 
     & \multicolumn{3}{c}{Number of resets} & \multicolumn{3}{c}{Distance walked between resets} & \multicolumn{3}{c}{Average alignment score}   \\ \hline
        Redirection Controller & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper  \\ \hline \hline
        S2C \cite{hodgson2013comparing} vs. ARC & 17.550 & 14.276 & 20.824 & -12.458 & -15.417 & -9.500 & 0.871 & 0.858 & 0.883  \\ \hline
        APF \cite{thomas2019general} vs ARC & 5.417 & 2.549 & 8.284 & -6.599 & -9.476 & -3.722 & 0.073 & 0.058 & 0.088  \\ \hline
        S2C \cite{hodgson2013comparing} vs 
        APF \cite{thomas2019general} & 11.617 & 9.148 & 14.086 & -5.822 & -6.808 & -4.836 & 0.801 & 0.789 & 0.813  \\
    \multicolumn{10}{c}{}    \\ 
    \multicolumn{10}{c}{\textbf{Environment B}}    \\ 
     & \multicolumn{3}{c}{Number of resets} & \multicolumn{3}{c}{Distance walked between resets} & \multicolumn{3}{c}{Average alignment score}   \\ \hline
        Redirection Controller & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper  \\ \hline \hline
        S2C \cite{hodgson2013comparing} vs. ARC & 46.867 & 32.784 & 60.950 & -0.507 & -0.630 & -0.385 & 0.808 & 0.778 & 0.838  \\ \hline
        APF \cite{thomas2019general} vs ARC & 11.317 & 3.449 & 19.184 & -0.130 & -0.237 & -0.023 & 0.761 & 0.747 & 0.774  \\ \hline
        S2C \cite{hodgson2013comparing} vs 
        APF \cite{thomas2019general} & 36.408 & 23.560 & 49.256 & -0.382 & -0.502 & -0.263 & 0.033 & 0.002 & 0.065  \\
    \multicolumn{10}{c}{}    \\ 
    \multicolumn{10}{c}{\textbf{Environment C}}    \\ 
     & \multicolumn{3}{c}{Number of resets} & \multicolumn{3}{c}{Distance walked between resets} & \multicolumn{3}{c}{Average alignment score}   \\ \hline
        Redirection Controller & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper  \\ \hline \hline
        S2C \cite{hodgson2013comparing} vs. ARC & 2139.983 & 2062.215 & 2217.752 & -3.719 & -3.792 & -3.645 & -1.036 & -1.060 & -1.012  \\ \hline
        APF \cite{thomas2019general} vs ARC & 137.108 & 124.065 & 150.152 & -2.296 & -2.420 & -2.171 & -0.109 & -0.131 & -0.087  \\ \hline
        S2C \cite{hodgson2013comparing} vs 
        APF \cite{thomas2019general} & 2005.500 & 1928.841 & 2082.159 & -1.414 & -1.488 & -1.339 & -0.928 & -0.961 & -0.894  \\
    \end{tabular}
    \caption{The results of pairwise post-hoc comparisons between controllers, computed using linear contrasts and reported using confidence intervals due to the large sample size \cite{lin2013research}. For each metric, $\hat{\psi}$ is the difference in estimated means between the two groups (estimate of the true mean). CI lower is the lower bound of the confidence interval on this difference, and CI upper is the upper bound. Narrower intervals indicate a more precise estimate of the true mean. We can interpret a cell as the estimated difference between the group means ($\hat{\psi}$), and CI lower and CI upper to represent that on $95\%$ of samples, the true difference in means between the groups will fall in the range $[\hat{\psi} - \text{CI lower}, \hat{\psi} + \text{CI upper}]$. For a given row that compares Algorithm X vs. Algorithm Y, a positive $\hat{\psi}$ value indicates that Algorithm X scored more than Algorithm Y by that $\hat{\psi}$, while negative a value indicates that Algorithm X scored lower than Algorithm Y by that $\hat{\psi}$, bounded by CI lower and CI upper.}
    \label{tab:results}
\end{table*}

% - we replaced outliers with the median value to make comparisons more robust (rdw can be succeptible to outliers)
% - normality was tested using qq plots, histograms, and measure of skewness and kurtosis. large sample size makes the norm test unreliable (shapiro wilks? don't remember the name)
% - we report confidence intervals because large sample size (only 100 paths, but each path has a lot of data). also, CIs is better for comparing against other research if they also report CIs. \cite{lin2013research}
% - i shoudl report my p values as p<0.001 when R tells me they are p=0
% - the degrees of freedom in the ANOVA are not integers because sphericity is violated, and the function automatically does a correctoion to account for this, which makes the DoF smaller than normal

\subsection{Experiment 1} \label{sec:exp1}
\label{results:exp1}
Experiment 1 was conducted in Environment A.
\subsubsection{Number of resets}
The robust repeated-measures ANOVA revealed a significant effect of redirection controller on the number of resets in Environment A $F(1.67,98.28)=133.2998$.
A boxplot of the number of resets incurred by each controller across all trials is shown in \autoref{fig:envA_resets}, and the results of post-hoc tests are shown in \autoref{tab:results}.

ARC outperformed both S2C and APF as it was usually able to steer the user on the same virtual path as S2C and APF, but with fewer collisions.
ARC sometimes performed worse than APF, as indicated by the long upper whisker in \autoref{fig:envA_resets}.
However, ARC was also sometimes able to achieve perfect alignment and steer users along paths with no collisions, which APF and S2C were not able to do.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\linewidth]{img/envA_resets.png}
    \caption{The number of resets for each redirection controller in Environment A. The boxplots show the median and IQR for the data. A significant difference was found between all algorithms. ARC resulted in significantly fewer collisions with the physical environment than APF and S2C did.}
    \label{fig:envA_resets}
\end{figure}

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
There was a significant effect of controller on the distance walked $F(1.15,68.06)=71.8013, p<.0001$.
A boxplot of the average distance walked between resets for each controller is shown in \autoref{fig:envA_distance}, and the precise difference between controllers is shown in \autoref{tab:results}.

When navigating with ARC, the user was able to walk further without colliding with a physical obstacle when compared against APF and S2C.
The long upper whisker and the dots representing outlier paths indicate that for some paths, the simulated user was able to walk over $45m$ before colliding with an obstacle, which shows that ARC is able to deliver VR experiences with a lot of locomotion and very few resets.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envA_distance.png}
    \caption{The average distance walked between resets for each path with each controller in Environment A. Significant differences were found between all controllers. On average, ARC allowed the user to walk further before being reset due to a collision. The average distance for some paths is quite high because ARC was able to achieve alignment and steer the user along a collision-free path.}
    \label{fig:envA_distance}
\end{figure}

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The robust trimmed means ANOVA revealed a significant effect of steering controller on the user's average alignment $F(1.98,117.08)=17156.3,p<.0001$.
The distribution of average distance walked between resets across all trials is shown in \autoref{fig:envA_alignment}, and the differences between group means can be found in \autoref{tab:results}.

The user's average alignment score was usually lower when they were redirected with ARC than when they were redirected with either APF or S2C.
Neither APF nor S2C is designed using concepts of alignment, so they should not be expected to achieve higher alignment scores than ARC is.
The fairly short whiskers in \autoref{fig:envA_alignment} indicates that the user's alignment was consistently low regardless of the path, which signals to some reliability of ARC to make the state at least close to aligned.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envA_alignment.png}
    \caption{The average alignment for the user in Environment A when steered with each controller. As expected, ARC maintained a low alignment score, while S2C and APF did not. Alignment measures the difference between the user's physical and virtual states, so a lower alignment is better.}
    \label{fig:envA_alignment}
\end{figure}

\subsubsection{Qualitative Evaluations}
The heat map of the physical space for Environment A is shown in \autoref{fig:envA_combined_heatmap}.
Every controller had the user spend most of their time near the center of the environment.
This is what S2C is designed to do, and APF reduces to S2C in empty environments, so this is no surprise.
One interesting thing to note, however, is that when the user is steered using ARC, they spend less time at the center of the room compared to S2C and APF.

\autoref{fig:resets_by_CR} shows that in Environment A, S2C is outperformed by APF and ARC, and APF is outperformed by ARC.
The differences in performance are fairly even, although S2C is very slightly worse than APF than APF is compared to ARC.
% This is because ARC is able to steer the user on collision-free paths if the physical and virtual states are close enough that ARC can cause the system to become perfectly aligned.
% Once this happens, redirection is no longer needed since the PE and VE are identical.
% This never happens with S2C or APF.

The frequency plot of the average curvature gains applied by each controller across all 100 paths is shown in \autoref{fig:envA_steering}.
The implementation of APF we used \cite{thomas2019general} always applies maximum curvature gain.
However, S2C and ARC do not always apply the maximum curvature gain.
The average curvature gain for each path steered by S2C is always above $6^\circ$, which is still fairly high considering the perceptual limit is about $7.6^\circ$.
On the other hand, ARC is able to apply curvature gains much lower than the perceptual limit and with high consistency, mostly ranging from $3^\circ/s$ to $6^\circ/s$.
All of the average gains applied by ARC are below $7^\circ$, and they are nicely distributed across the whole range of possible gains.
This shows that ARC applies less intense gains much more often than other controllers, which creates a more comfortable experience for the user.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envA_combined_heatmap.pdf}
    \caption{A heat map of the user's physical position across all paths for each controller in Environment A. Yellow tiles indicate the most time spent at that location, while purple tiles indicate the least amount of time. S2C and APF steer the user such that they spent the large majority of their time in the center of the room, while ARC allows the user to visit each region of the room more evenly.}
    \label{fig:envA_combined_heatmap}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envA_steering_rate_short.png}
    \caption{A histogram of the average curvature gain applied by each controller for each path in Environment A. The implementation of APF we used always applies the same gain, while S2C and ARC apply lower gains on average. S2C still applies gains fairly close to the perceptual threshold ($\approx 7.6^\circ /s$), but ARC is able to steer the user on paths with fewer collisions and significantly reduced curvature gains. Most of the gains applied by ARC fall in the $3^\circ/s - 5^\circ /s$ range, showing that ARC only applies the gains necessary to avoid collisions and maintain alignment.}
    \label{fig:envA_steering}
\end{figure}

\subsection{Experiment 2} \label{sec:exp2}
Experiment 2 was conducted in Environment B.
\subsubsection{Number of resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The robust ANOVA revealed a significant effect of controller on the number of resets $F(1.6,94.42)=56.0129,p<.0001$.
The boxplot showing the distribution of number of resets across all paths for each steering controller is shown in \autoref{fig:envB_resets}, and the results from pairwise post-hoc tests are shown in \autoref{tab:results}.

As can be seen in \autoref{fig:envB_resets}, ARC and APF have somewhat similar performances, although ARC still resulted in significantly fewer resets than APF did.
Furthermore, the interquartile range for the number of resets is lower for ARC than it is for APF, which provides evidence in support of the notion that ARC is able to deliver a consistent locomotion experience that is robust to different virtual paths.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_resets.png}
    \caption{The number of resets across all paths for each redirection controller in Environment B. ARC and APF have somewhat similar performance, but ARC still achieves a lower spread and median number of resets than APF. S2C performs much worse than ARC and APF due to the obstacles placed in the physical room (see \autoref{fig:environments}).}
    \label{fig:envB_resets}
\end{figure}

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
There was a significant effect of steering algorithm on the average distance walked between resets $F(1.9,112.05)=58.9188 ,p<.0001$.
A plot of the average distances walked between resets for all paths with all controllers is shown in \autoref{fig:envB_distance}.
The results of post-hoc tests to determine the precise differences between controllers is shown in \autoref{tab:results}.

The boxplot for the physical distances walked in Environment B show that ARC achieves a higher median distance than APF and S2C, but the largest average distances afforded by ARC are not as long as the longest distances walked with APF.
This is similar to the trend seen in the number of resets (\autoref{fig:envB_resets}), where ARC performs significantly better than APF, but the absolute best cases for APF yield a better performance than the best cases for ARC.
This suggests that APF may be more suited than ARC for navigation in environments will corridors, like Environment B, but additional studies should be conducted to confirm this.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_distance.png}
    \caption{The average physical distance walked between resets across all paths for each controller in Environment B. We see a similar pattern to the number of resets, wherein ARC and APF have similar performances with ARC achieving a higher distance walked, and S2C performs poorly and often requires resets after walking less than $1m$, as indicated by the long whiskers of the purple boxplot.}
    \label{fig:envB_distance}
\end{figure}

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A significant effect of redirection controller on the user's average alignment was found $F(1.44,84.85)=3484.467,p<.0001$.
The average alignment scores for all controllers in Environment B are shown in \autoref{fig:envB_alignment}, and the results from post-hoc comparisons can be found in \autoref{tab:results}.

The same trend as was seen in Environment A for the average alignment score across all paths is seen in Environment B as well.
ARC achieves a noticeably lower alignment score, which shows that ARC is able to successfully steer the user to a more aligned state (perfect alignment yields a score of 0).
Significant differences in alignment scores were found between APF and S2C (just as they were in Environment A).
% , but we do not believe this is a particularly interesting comparison to make since both controllers are not designed with alignment in mind; the important comparison is between ARC and the other two controllers.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_alignment.png}
    \caption{Average alignment score of the user over all paths in Environment B, for all redirection controllers. ARC is able to maintain a relatively low alignment score (a score of 0 indicates perfect alignment), while S2C and APF exhibit higher alignment scores. This is not unexpected since APF and S2C are not designed using alignment, but it indicates that ARC is working as intended.}
    \label{fig:envB_alignment}
\end{figure}

\subsubsection{Qualitative Evaluations}
The heat map showing the user's occupancy in the physical space for Environment B is shown in \autoref{fig:envB_combined_heatmap}.
S2C and APF have very similar heat maps since both algorithms steer the user towards the center of the space.
APF steers the user towards the center \textit{not} because it reduces to S2C, as it did in Environment A, but because the center of Environment B is the most open space in the environment, furthest away from all obstacles.
The heat map for ARC is very interesting.
While the user is able to visit most areas of the room, there is a clear tendency to keep the user in the upper-left corner of the room.
It is possible that ARC is getting stuck, which is not particularly surprising in this constrained environment, but it is interesting that there is a bias towards one side of the room, rather than ARC getting the user stuck equally across the room.
The reason for this is not clear, and further work should be done to better understand biases like this.

The number of resets for each algorithm in Environment B are compared in \autoref{fig:resets_by_CR}.
As expected, the number of resets increases for all controllers, since Environment B is more complex than Environment A.
Interestingly, however, the difference in performance between ARC and the other algorithms is much smaller than it was in Environment A.
This is likely related to ARC's tendency to steer the user near the top wall, but it is possible that there is another reason for ARC's relatively worse performance versus its performance in Environment A.

\autoref{fig:envB_steering} shows the average curvature gain applied by each controller over all paths in Environment B.
Much like Environment A, S2C and ARC apply weaker gains than APF.
One difference between Environment A and B is that ARC applies stronger gains more often than S2C.
The spread of gains applied by ARC is also much smaller than it was in Environment A, which is likely because ARC was not able to achieve perfect alignment and thus was not able to apply weak gains while also lowering the user's alignment score.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_combined_heatmap.pdf}
    \caption{A heat map of the physical locations visited by the user in Environment B when steered with each controller. Yellow tiles indicate more visits to a region, while purple tiles indicate less time spent in a region. Obstacles are shown in black. S2C and APF keep the user concentrated near the center of the room since it is the most open space in all directions, while ARC is able to utilize more of the space and steer the user along all corridors in the room. ARC has some tendency to keep the user near the north wall of the room, which we suspect is due to the user getting stuck in between obstacles, but the exact cause is not clear.}
    \label{fig:envB_combined_heatmap}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_steering_rate_short.png}
    \caption{A histogram of the average curvature gain applied for each path with each controller in Environment B. As in Environment A, APF applies a constant curvature gain when the user is walking. S2C and ARC apply gains with an average in the range of $4^\circ/s - 6^\circ/s$, with ARC applying gains all gains at a lower intensity than about half of the gains applied by S2C. Note that the lowest gains applied by S2C are lower than those of ARC.}
    \label{fig:envB_steering}
\end{figure}

\subsection{Experiment 3} \label{sec:exp3}
Experiment 3 was conduct in Environment C.
\subsubsection{Number of resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
There was a significant effect of controller on the number of resets $F(1.04,61.34)=4186.948,p<.0001$.
A boxplot of the number of collisions incurred in Environment C with all controllers on each path is shown in \autoref{fig:envC_resets}, and the differences in number of collisions between groups is shown in \autoref{tab:results}.
Note the log scale of the boxplot due to the high number of collisions S2C caused.

An interesting trend is seen in the number of collisions in Environment C.
ARC performs dramatically better than APF (and S2C, unsurprisingly), with a much smaller spread of number of collisions.
That is, ARC exhibits a very consistent ability to steer the user on paths.
Paths steered by APF all have at least as many collisions as paths steered by ARC, and are sometimes more than twice as bad as the worst path for ARC.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envC_resets.png}
    \caption{The number of resets on each path for each controller in Environment C. Again, S2C has a very poor performance, but this time it is due to the obstacle occupying the center of the room. ARC has a lower reset rate than APF, and also has a much lower variance in numbers of resets, indicating that in highly complex environments like Environment C ($CR = 0.562$), the user can be consistently steering with a relatively low number of resets.}
    \label{fig:envC_resets}
\end{figure}

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A robust trimmed-means ANOVA indicated a significant effect of controller on the average physical distance walked by the user between resets $F(1.52,89.44)=5855.824,p<.0001$.
Boxplots showing the distributions of average distances walked between resets for all controllers in Environment C is shown in \autoref{fig:envC_distance}, and the results from post-hoc significance tests are in \autoref{tab:results}.

As expected, we see the same pattern in the distance walked between resets as we did in the number of resets.
ARC outperforms APF and S2C, and the results for ARC are more consistent than they are for APF, though not as dramatic a difference as there was for the number of resets (see \textbf{[add reference to descriptive stats in supplementary materials]}).
This highlights the importance of using multiple metrics to evaluate and compare steering controllers.
The number of resets for Environment C shows that ARC performs much more consistently than APF, but the average distance between resets for Environment C, while it shows the same overall trend, suggests that the difference in consistency is not as large as it seemed from the number of resets.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envC_distance.png}
    \caption{Average distance walked between resets on each path for all controllers in Environment C. S2C has a poor performance due to being constantly reset and redirected back to the obstacle in the center of the room. APF allows the user to walk further than S2C does, but still often triggers a reset less than every $2m$. The long upper whisker on the APF boxplot indicates that APF can achieve decent performance on some paths. ARC is able to steer the user much further than APF on all paths, with a median distance walked between resets of $4m$.}
    \label{fig:envC_distance}
\end{figure}

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
We found a significant effect of steering controller on the user's average alignment $F(1.04,61.34)=4186.948,p<.0001$.
A plot of the average alignment score across 100 paths for all controllers is shown in \autoref{fig:envC_alignment}.
The post-hoc tests are in \autoref{tab:results}.

An interesting pattern seen in the alignment scores for Environment C is that S2C scores the best (lowest) average alignment of all the controllers, and ARC has the highest alignment score.
This is surprising since neither S2C nor APF is designed to work based on alignment, but ARC is.
Even though ARC has the worst average alignment score of all the controllers in Environment, it undoubtedly has the best performance in terms of number of collisions and physical distance travelled between resets.
This disagreement in the metrics suggests that the alignment metric we used in this study may not be a good representation of an alignment-based controller's ability to keep the system aligned and avoid collisions.
We stress that we \textit{do not} believe this means the alignment-based methods ARC uses to steer the user are flawed, since all other results in this section indicate that ARC \textit{does} work well in comparison to other controllers.
It may simply be the case that reporting the averaged sum of the user's forward and lateral alignment is not a good way to measure an controller's alignment capabilities, since the results from Environment C show that it is possible for a controller that does not use alignment to have a better alignment score.
Since this paper is only the second to formally study concepts of alignment, our alignment metric can likely be improved.
More work should be done to develop a metric for alignment that consistently reflects a controller's ability to keep a system aligned.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envC_alignment.png}
    \caption{The average alignment score for all paths with each controller in Environment C. Interestingly, S2C achieves the best (lowest) alignment score, despite have a very high number of resets and low travel distance between resets. ARC achieves an alignment score lower than APF, but worse than S2C. The reason for this is not clear, since S2C is not designed around alignment. This suggests that measuring alignment score may not be the most useful metric, since ARC is able to achieve much better performance than S2C, but still has a worse alignment score.}
    \label{fig:envC_alignment}
\end{figure}

\subsubsection{Qualitative Evaluations}
A heat map of the user in the physical space for Environment C is shown in \autoref{fig:teaser}.
% The black rectangles represent obstacles in the environment, and purple tiles indicate low frequency of the user being in that area, while yellow tiles indicate high frequency.
It is clear that ARC utilizes more of the PE for navigation than do APF or S2C, but there is still a bias towards the leftmost region of the room.
This is similar to the bias seen in the heat map for ARC in Environment B, which suggests that this may not be a product of random chance and that ARC prefers to steer the user to a particular region of the PE.
% We saw a bias in the user's position when using ARC in both Environment B and C, which suggests that there is something going on that is causing ARC to prefer parts of the room over others.
Visual inspection of the random starting positions in the PE confirmed that the bias was not due to the starting position, so more work should be done to get a better understanding of the biases of ARC.

% APF does worse than ARC at using all of the space available in the PE, with the user being concentrated mostly in the open space in the bottom region of the room.
% The user is able to walk through the other regions in the room sometimes, but the algorithm shows a clear bias towards the largest free space in the room.
% S2C performs very poorly, since there is an obstacle in the center of the physical room.
% The user is constantly redirected towards the center, only to be turned away when they get too close, and then steered right back to the center.
% The high concentration near the center of the room is supported by the very high number of resets they incurred in this space (see \autoref{fig:envC_resets}).

The performance of ARC, APF, and S2C is also compared in \autoref{fig:resets_by_CR}.
ARC achieves much fewer resets than either APF or S2C in Environment C, which is the most complex, which highlights ARC's ability to handle physical and virtual environments with differing configurations and complexities.
Interestingly, the performance of ARC increases going from Environment B to Environment C, which suggests that in addition to the complexity metric we used (measure of relative proximity to obstacles in the PE and VE), the shapes of the free space may be important for an algorithm's performance.
% It should also be noted that APF and S2C do not see this same increase in performance from Environment B to C, and both consistently get worse as the complexity increases, as one would expect.
% This shows that our novel complexity metric is still useful for assessing controller performance in complex environments.

Finally, \autoref{fig:envC_steering} shows a frequency plot of the gains applied by each controller across all paths in Environment C.
All gains applied by both ARC and S2C are lower than that of APF, with ARC applying the lowest gains of all, and applying stronger gains less often than S2C.
This highlights one of the major strength of our algorithm: ARC is able to achieve a lower number of resets than current state of the art while also applying \textit{less intense} gains.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/resets_by_CR.png}
    \caption{The relationship between the environment complexity and the number of resets incurred by a redirection controller. ARC consistently has a better performance than S2C and APF for all environment complexities. The performance difference between ARC and the other algorithms is quite large for environments A and C, but the difference decreases drastically for Environment B. It is not clear why Environment B causes the controllers to have a more similar performance, but it may be due to the relatively few pathing options afforded by the narrow hallways of Environment B. Environments A and C both include regions with a fairly large amount of open space, unlike Environment B (see \autoref{fig:environments}).}
    \label{fig:resets_by_CR}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envC_steering_rate_short.png}
    \caption{The average curvature gain applied by each controller for all paths in Environment C. The same trend as in Environment B is seen here, where APF has a higher steering rate than S2C and ARC. One difference between the steering rates in Environment B and C is that the gains applied by S2C and ARC are in a higher range ($6^\circ/s - 7^\circ/s$) in Environment C than they were in Environment B ($4^\circ/s - 6^\circ/s$).}
    \label{fig:envC_steering}
\end{figure}


==> results3.tex <==
\section{Results} \label{results}
We performed evaluations of the performance of S2C, APF, and ARC using three quantitative metrics and three qualitative metrics (\autoref{subsec:evaluation}).
Each of the metrics was computed for all 100 paths in each condition.
In complex environments, RDW controller algorithms can sometimes encounter ``unlucky'' virtual paths that make it particularly difficult to avoid collisions, and the user will end up incurring many collisions in a small time frame.
% (they essentially get ``stuck'' on an obstacle).
To make our comparisons robust to these unlucky paths, outliers in the data that were $1.5$ times larger than the interquartile range of the data were replaced with the median of the data.
We evaluated the normality of the data using visual inspection of Q-Q plots and histograms as well as measures of the distributions' skew and kurtosis.
Homoscedasticity was evaluated using Levene's test.
For each metric measured, the assumption of normality or homoscedasticity was violated, so we conducted all of our tests using a robust one-way repeated measures $20\%$ trimmed means ANOVA (using the WRS2 package for R).
Pairwise post-hoc comparisons were computed using linear contrasts.

Due to the large sample size in our experiments, we report $95\%$ confidence interval instead of \textit{p}-values.
As the sample size grows, statistical tests become sensitive to small differences between samples, and the \textit{p}-value becomes unreliable as it approaches $0$.
Confidence intervals, however, become narrower as the sample size grows, which means they are able to scale with the sample size and are still reliable for experiments with large samples.
Furthermore, reporting confidence intervals allows for easier comparisons with future work if they also report confidence intervals, since the interval provides numerical bounds on the differences between conditions \cite{lin2013research}.

The results are shown in \autoref{tab:results}, with discussions in subsequent sections.
Most of the discussion is limited to comparing ARC to APF, since it is already well-established that APF outperforms S2C \cite{thomas2019general, bachmann2019multi}.
A confidence interval that does not contain 0 in its range [CI lower, CI upper] is considered to be significant.
Thus, we found significant differences between all groups in our post-hoc tests.
The common pattern seen in the results is that ARC outperforms APF and S2C, while APF outperforms S2C.
One condition for which this was not the case is the alignment metric in Environment C.
% Full descriptive statistics for each metric for each controller are in the supplemental materials \autoref{}.

% \textbf{[need to mention that the alignment comparison between APF and S2C doesn't make sense since neiter algortihm considers alignment. maybe put it in the metrics section of section 4?]}

\begin{table*}[ht]
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
    \multicolumn{10}{c}{\textbf{Environment A}}    \\ 
     & \multicolumn{3}{c}{Number of resets} & \multicolumn{3}{c}{Distance walked between resets} & \multicolumn{3}{c}{Average alignment score}   \\ \hline
        Redirection Controller & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper  \\ \hline \hline
        S2C \cite{hodgson2013comparing} vs. ARC & 17.550 & 14.276 & 20.824 & -12.458 & -15.417 & -9.500 & 0.871 & 0.858 & 0.883  \\ \hline
        APF \cite{thomas2019general} vs ARC & 5.417 & 2.549 & 8.284 & -6.599 & -9.476 & -3.722 & 0.073 & 0.058 & 0.088  \\ \hline
        S2C \cite{hodgson2013comparing} vs 
        APF \cite{thomas2019general} & 11.617 & 9.148 & 14.086 & -5.822 & -6.808 & -4.836 & 0.801 & 0.789 & 0.813  \\
    \multicolumn{10}{c}{}    \\ 
    \multicolumn{10}{c}{\textbf{Environment B}}    \\ 
     & \multicolumn{3}{c}{Number of resets} & \multicolumn{3}{c}{Distance walked between resets} & \multicolumn{3}{c}{Average alignment score}   \\ \hline
        Redirection Controller & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper  \\ \hline \hline
        S2C \cite{hodgson2013comparing} vs. ARC & 46.867 & 32.784 & 60.950 & -0.507 & -0.630 & -0.385 & 0.808 & 0.778 & 0.838  \\ \hline
        APF \cite{thomas2019general} vs ARC & 11.317 & 3.449 & 19.184 & -0.130 & -0.237 & -0.023 & 0.761 & 0.747 & 0.774  \\ \hline
        S2C \cite{hodgson2013comparing} vs 
        APF \cite{thomas2019general} & 36.408 & 23.560 & 49.256 & -0.382 & -0.502 & -0.263 & 0.033 & 0.002 & 0.065  \\
    \multicolumn{10}{c}{}    \\ 
    \multicolumn{10}{c}{\textbf{Environment C}}    \\ 
     & \multicolumn{3}{c}{Number of resets} & \multicolumn{3}{c}{Distance walked between resets} & \multicolumn{3}{c}{Average alignment score}   \\ \hline
        Redirection Controller & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper & $\hat{\psi}$ & CI lower & CI upper  \\ \hline \hline
        S2C \cite{hodgson2013comparing} vs. ARC & 2139.983 & 2062.215 & 2217.752 & -3.719 & -3.792 & -3.645 & -1.036 & -1.060 & -1.012  \\ \hline
        APF \cite{thomas2019general} vs ARC & 137.108 & 124.065 & 150.152 & -2.296 & -2.420 & -2.171 & -0.109 & -0.131 & -0.087  \\ \hline
        S2C \cite{hodgson2013comparing} vs 
        APF \cite{thomas2019general} & 2005.500 & 1928.841 & 2082.159 & -1.414 & -1.488 & -1.339 & -0.928 & -0.961 & -0.894  \\
    \end{tabular}
    \caption{The results of pairwise post-hoc comparisons between controllers, computed using linear contrasts and reported using confidence intervals due to the large sample size \cite{lin2013research}. For each metric, $\hat{\psi}$ is the difference in estimated means between the two groups (estimate of the true mean). CI lower is the lower bound of the confidence interval on this difference, and CI upper is the upper bound. Narrower intervals indicate a more precise estimate of the true mean. We can interpret a cell as the estimated difference between the group means ($\hat{\psi}$), and CI lower and CI upper to represent that on $95\%$ of samples, the true difference in means between the groups will fall in the range $[\hat{\psi} - \text{CI lower}, \hat{\psi} + \text{CI upper}]$. For a given row that compares Algorithm X vs. Algorithm Y, a positive $\hat{\psi}$ value indicates that Algorithm X scored more than Algorithm Y by that $\hat{\psi}$, while negative a value indicates that Algorithm X scored lower than Algorithm Y by that $\hat{\psi}$, bounded by CI lower and CI upper.}
    \label{tab:results}
\end{table*}

% - we replaced outliers with the median value to make comparisons more robust (rdw can be succeptible to outliers)
% - normality was tested using qq plots, histograms, and measure of skewness and kurtosis. large sample size makes the norm test unreliable (shapiro wilks? don't remember the name)
% - we report confidence intervals because large sample size (only 100 paths, but each path has a lot of data). also, CIs is better for comparing against other research if they also report CIs. \cite{lin2013research}
% - i shoudl report my p values as p<0.001 when R tells me they are p=0
% - the degrees of freedom in the ANOVA are not integers because sphericity is violated, and the function automatically does a correctoion to account for this, which makes the DoF smaller than normal

\begin{figure*}[t]
    \centering
    \includegraphics[width=.9\linewidth]{img/all_boxplots.png}
    \caption{The number of resets for each redirection controller in Environment A. The boxplots show the median and IQR for the data. A significant difference was found between all algorithms. ARC resulted in significantly fewer collisions with the physical environment than APF and S2C did.}
    \label{fig:envA_resets}
\end{figure*}

\subsection{Experiment 1} \label{sec:exp1}
\label{results:exp1}
Experiment 1 was conducted in Environment A.
\subsubsection{Number of resets}
The robust repeated-measures ANOVA revealed a significant effect of redirection controller on the number of resets in Environment A $F(1.67,98.28)=133.2998$.
A boxplot of the number of resets incurred by each controller across all trials is shown in \autoref{fig:envA_resets}, and the results of post-hoc tests are shown in \autoref{tab:results}.

ARC outperformed both S2C and APF as it was usually able to steer the user on the same virtual path as S2C and APF, but with fewer collisions.
ARC sometimes performed worse than APF, as indicated by the long upper whisker in \autoref{fig:envA_resets}.
However, ARC was also sometimes able to achieve perfect alignment and steer users along paths with no collisions, which APF and S2C were not able to do.

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
There was a significant effect of controller on the distance walked $F(1.15,68.06)=71.8013, p<.0001$.
A boxplot of the average distance walked between resets for each controller is shown in \autoref{fig:envA_distance}, and the precise difference between controllers is shown in \autoref{tab:results}.

When navigating with ARC, the user was able to walk further without colliding with a physical obstacle when compared against APF and S2C.
The long upper whisker and the dots representing outlier paths indicate that for some paths, the simulated user was able to walk over $45m$ before colliding with an obstacle, which shows that ARC is able to deliver VR experiences with a lot of locomotion and very few resets.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envA_distance.png}
%     \caption{The average distance walked between resets for each path with each controller in Environment A. Significant differences were found between all controllers. On average, ARC allowed the user to walk further before being reset due to a collision. The average distance for some paths is quite high because ARC was able to achieve alignment and steer the user along a collision-free path.}
%     \label{fig:envA_distance}
% \end{figure}

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The robust trimmed means ANOVA revealed a significant effect of steering controller on the user's average alignment $F(1.98,117.08)=17156.3,p<.0001$.
The distribution of average distance walked between resets across all trials is shown in \autoref{fig:envA_alignment}, and the differences between group means can be found in \autoref{tab:results}.

The user's average alignment score was usually lower when they were redirected with ARC than when they were redirected with either APF or S2C.
Neither APF nor S2C is designed using concepts of alignment, so they should not be expected to achieve higher alignment scores than ARC is.
The fairly short whiskers in \autoref{fig:envA_alignment} indicates that the user's alignment was consistently low regardless of the path, which signals to some reliability of ARC to make the state at least close to aligned.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envA_alignment.png}
%     \caption{The average alignment for the user in Environment A when steered with each controller. As expected, ARC maintained a low alignment score, while S2C and APF did not. Alignment measures the difference between the user's physical and virtual states, so a lower alignment is better.}
%     \label{fig:envA_alignment}
% \end{figure}

\subsubsection{Qualitative Evaluations}
The heat map of the physical space for Environment A is shown in \autoref{fig:envA_combined_heatmap}.
Every controller had the user spend most of their time near the center of the environment.
This is what S2C is designed to do, and APF reduces to S2C in empty environments, so this is no surprise.
One interesting thing to note, however, is that when the user is steered using ARC, they spend less time at the center of the room compared to S2C and APF.

\autoref{fig:resets_by_CR} shows that in Environment A, S2C is outperformed by APF and ARC, and APF is outperformed by ARC.
The differences in performance are fairly even, although S2C is very slightly worse than APF than APF is compared to ARC.
% This is because ARC is able to steer the user on collision-free paths if the physical and virtual states are close enough that ARC can cause the system to become perfectly aligned.
% Once this happens, redirection is no longer needed since the PE and VE are identical.
% This never happens with S2C or APF.

The frequency plot of the average curvature gains applied by each controller across all 100 paths is shown in \autoref{fig:envA_steering}.
The implementation of APF we used \cite{thomas2019general} always applies maximum curvature gain.
However, S2C and ARC do not always apply the maximum curvature gain.
The average curvature gain for each path steered by S2C is always above $6^\circ$, which is still fairly high considering the perceptual limit is about $7.6^\circ$.
On the other hand, ARC is able to apply curvature gains much lower than the perceptual limit and with high consistency, mostly ranging from $3^\circ/s$ to $6^\circ/s$.
All of the average gains applied by ARC are below $7^\circ$, and they are nicely distributed across the whole range of possible gains.
This shows that ARC applies less intense gains much more often than other controllers, which creates a more comfortable experience for the user.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envA_combined_heatmap.pdf}
    \caption{A heat map of the user's physical position across all paths for each controller in Environment A. Yellow tiles indicate the most time spent at that location, while purple tiles indicate the least amount of time. S2C and APF steer the user such that they spent the large majority of their time in the center of the room, while ARC allows the user to visit each region of the room more evenly.}
    \label{fig:envA_combined_heatmap}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envA_steering_rate_short.png}
    \caption{A histogram of the average curvature gain applied by each controller for each path in Environment A. The implementation of APF we used always applies the same gain, while S2C and ARC apply lower gains on average. S2C still applies gains fairly close to the perceptual threshold ($\approx 7.6^\circ /s$), but ARC is able to steer the user on paths with fewer collisions and significantly reduced curvature gains. Most of the gains applied by ARC fall in the $3^\circ/s - 5^\circ /s$ range, showing that ARC only applies the gains necessary to avoid collisions and maintain alignment.}
    \label{fig:envA_steering}
\end{figure}

\subsection{Experiment 2} \label{sec:exp2}
Experiment 2 was conducted in Environment B.
\subsubsection{Number of resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
The robust ANOVA revealed a significant effect of controller on the number of resets $F(1.6,94.42)=56.0129,p<.0001$.
The boxplot showing the distribution of number of resets across all paths for each steering controller is shown in \autoref{fig:envB_resets}, and the results from pairwise post-hoc tests are shown in \autoref{tab:results}.

As can be seen in \autoref{fig:envB_resets}, ARC and APF have somewhat similar performances, although ARC still resulted in significantly fewer resets than APF did.
Furthermore, the interquartile range for the number of resets is lower for ARC than it is for APF, which provides evidence in support of the notion that ARC is able to deliver a consistent locomotion experience that is robust to different virtual paths.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envB_resets.png}
%     \caption{The number of resets across all paths for each redirection controller in Environment B. ARC and APF have somewhat similar performance, but ARC still achieves a lower spread and median number of resets than APF. S2C performs much worse than ARC and APF due to the obstacles placed in the physical room (see \autoref{fig:environments}).}
%     \label{fig:envB_resets}
% \end{figure}

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
There was a significant effect of steering algorithm on the average distance walked between resets $F(1.9,112.05)=58.9188 ,p<.0001$.
A plot of the average distances walked between resets for all paths with all controllers is shown in \autoref{fig:envB_distance}.
The results of post-hoc tests to determine the precise differences between controllers is shown in \autoref{tab:results}.

The boxplot for the physical distances walked in Environment B show that ARC achieves a higher median distance than APF and S2C, but the largest average distances afforded by ARC are not as long as the longest distances walked with APF.
This is similar to the trend seen in the number of resets (\autoref{fig:envB_resets}), where ARC performs significantly better than APF, but the absolute best cases for APF yield a better performance than the best cases for ARC.
This suggests that APF may be more suited than ARC for navigation in environments will corridors, like Environment B, but additional studies should be conducted to confirm this.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envB_distance.png}
%     \caption{The average physical distance walked between resets across all paths for each controller in Environment B. We see a similar pattern to the number of resets, wherein ARC and APF have similar performances with ARC achieving a higher distance walked, and S2C performs poorly and often requires resets after walking less than $1m$, as indicated by the long whiskers of the purple boxplot.}
%     \label{fig:envB_distance}
% \end{figure}

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A significant effect of redirection controller on the user's average alignment was found $F(1.44,84.85)=3484.467,p<.0001$.
The average alignment scores for all controllers in Environment B are shown in \autoref{fig:envB_alignment}, and the results from post-hoc comparisons can be found in \autoref{tab:results}.

The same trend as was seen in Environment A for the average alignment score across all paths is seen in Environment B as well.
ARC achieves a noticeably lower alignment score, which shows that ARC is able to successfully steer the user to a more aligned state (perfect alignment yields a score of 0).
Significant differences in alignment scores were found between APF and S2C (just as they were in Environment A).
% , but we do not believe this is a particularly interesting comparison to make since both controllers are not designed with alignment in mind; the important comparison is between ARC and the other two controllers.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envB_alignment.png}
%     \caption{Average alignment score of the user over all paths in Environment B, for all redirection controllers. ARC is able to maintain a relatively low alignment score (a score of 0 indicates perfect alignment), while S2C and APF exhibit higher alignment scores. This is not unexpected since APF and S2C are not designed using alignment, but it indicates that ARC is working as intended.}
%     \label{fig:envB_alignment}
% \end{figure}

\subsubsection{Qualitative Evaluations}
The heat map showing the user's occupancy in the physical space for Environment B is shown in \autoref{fig:envB_combined_heatmap}.
S2C and APF have very similar heat maps since both algorithms steer the user towards the center of the space.
APF steers the user towards the center \textit{not} because it reduces to S2C, as it did in Environment A, but because the center of Environment B is the most open space in the environment, furthest away from all obstacles.
The heat map for ARC is very interesting.
While the user is able to visit most areas of the room, there is a clear tendency to keep the user in the upper-left corner of the room.
It is possible that ARC is getting stuck, which is not particularly surprising in this constrained environment, but it is interesting that there is a bias towards one side of the room, rather than ARC getting the user stuck equally across the room.
The reason for this is not clear, and further work should be done to better understand biases like this.

The number of resets for each algorithm in Environment B are compared in \autoref{fig:resets_by_CR}.
As expected, the number of resets increases for all controllers, since Environment B is more complex than Environment A.
Interestingly, however, the difference in performance between ARC and the other algorithms is much smaller than it was in Environment A.
This is likely related to ARC's tendency to steer the user near the top wall, but it is possible that there is another reason for ARC's relatively worse performance versus its performance in Environment A.

\autoref{fig:envB_steering} shows the average curvature gain applied by each controller over all paths in Environment B.
Much like Environment A, S2C and ARC apply weaker gains than APF.
One difference between Environment A and B is that ARC applies stronger gains more often than S2C.
The spread of gains applied by ARC is also much smaller than it was in Environment A, which is likely because ARC was not able to achieve perfect alignment and thus was not able to apply weak gains while also lowering the user's alignment score.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_combined_heatmap.pdf}
    \caption{A heat map of the physical locations visited by the user in Environment B when steered with each controller. Yellow tiles indicate more visits to a region, while purple tiles indicate less time spent in a region. Obstacles are shown in black. S2C and APF keep the user concentrated near the center of the room since it is the most open space in all directions, while ARC is able to utilize more of the space and steer the user along all corridors in the room. ARC has some tendency to keep the user near the north wall of the room, which we suspect is due to the user getting stuck in between obstacles, but the exact cause is not clear.}
    \label{fig:envB_combined_heatmap}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envB_steering_rate_short.png}
    \caption{A histogram of the average curvature gain applied for each path with each controller in Environment B. As in Environment A, APF applies a constant curvature gain when the user is walking. S2C and ARC apply gains with an average in the range of $4^\circ/s - 6^\circ/s$, with ARC applying gains all gains at a lower intensity than about half of the gains applied by S2C. Note that the lowest gains applied by S2C are lower than those of ARC.}
    \label{fig:envB_steering}
\end{figure}

\subsection{Experiment 3} \label{sec:exp3}
Experiment 3 was conduct in Environment C.
\subsubsection{Number of resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
There was a significant effect of controller on the number of resets $F(1.04,61.34)=4186.948,p<.0001$.
A boxplot of the number of collisions incurred in Environment C with all controllers on each path is shown in \autoref{fig:envC_resets}, and the differences in number of collisions between groups is shown in \autoref{tab:results}.
Note the log scale of the boxplot due to the high number of collisions S2C caused.

An interesting trend is seen in the number of collisions in Environment C.
ARC performs dramatically better than APF (and S2C, unsurprisingly), with a much smaller spread of number of collisions.
That is, ARC exhibits a very consistent ability to steer the user on paths.
Paths steered by APF all have at least as many collisions as paths steered by ARC, and are sometimes more than twice as bad as the worst path for ARC.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envC_resets.png}
%     \caption{The number of resets on each path for each controller in Environment C. Again, S2C has a very poor performance, but this time it is due to the obstacle occupying the center of the room. ARC has a lower reset rate than APF, and also has a much lower variance in numbers of resets, indicating that in highly complex environments like Environment C ($CR = 0.562$), the user can be consistently steering with a relatively low number of resets.}
%     \label{fig:envC_resets}
% \end{figure}

\subsubsection{Average distance walked between resets}
% $(\hat{\psi}=xxx \ [xxx, xx])$
A robust trimmed-means ANOVA indicated a significant effect of controller on the average physical distance walked by the user between resets $F(1.52,89.44)=5855.824,p<.0001$.
Boxplots showing the distributions of average distances walked between resets for all controllers in Environment C is shown in \autoref{fig:envC_distance}, and the results from post-hoc significance tests are in \autoref{tab:results}.

As expected, we see the same pattern in the distance walked between resets as we did in the number of resets.
ARC outperforms APF and S2C, and the results for ARC are more consistent than they are for APF, though not as dramatic a difference as there was for the number of resets (see \textbf{[add reference to descriptive stats in supplementary materials]}).
This highlights the importance of using multiple metrics to evaluate and compare steering controllers.
The number of resets for Environment C shows that ARC performs much more consistently than APF, but the average distance between resets for Environment C, while it shows the same overall trend, suggests that the difference in consistency is not as large as it seemed from the number of resets.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envC_distance.png}
%     \caption{Average distance walked between resets on each path for all controllers in Environment C. S2C has a poor performance due to being constantly reset and redirected back to the obstacle in the center of the room. APF allows the user to walk further than S2C does, but still often triggers a reset less than every $2m$. The long upper whisker on the APF boxplot indicates that APF can achieve decent performance on some paths. ARC is able to steer the user much further than APF on all paths, with a median distance walked between resets of $4m$.}
%     \label{fig:envC_distance}
% \end{figure}

\subsubsection{Average alignment}
% $(\hat{\psi}=xxx \ [xxx, xx])$
We found a significant effect of steering controller on the user's average alignment $F(1.04,61.34)=4186.948,p<.0001$.
A plot of the average alignment score across 100 paths for all controllers is shown in \autoref{fig:envC_alignment}.
The post-hoc tests are in \autoref{tab:results}.

An interesting pattern seen in the alignment scores for Environment C is that S2C scores the best (lowest) average alignment of all the controllers, and ARC has the highest alignment score.
This is surprising since neither S2C nor APF is designed to work based on alignment, but ARC is.
Even though ARC has the worst average alignment score of all the controllers in Environment, it undoubtedly has the best performance in terms of number of collisions and physical distance travelled between resets.
This disagreement in the metrics suggests that the alignment metric we used in this study may not be a good representation of an alignment-based controller's ability to keep the system aligned and avoid collisions.
We stress that we \textit{do not} believe this means the alignment-based methods ARC uses to steer the user are flawed, since all other results in this section indicate that ARC \textit{does} work well in comparison to other controllers.
It may simply be the case that reporting the averaged sum of the user's forward and lateral alignment is not a good way to measure an controller's alignment capabilities, since the results from Environment C show that it is possible for a controller that does not use alignment to have a better alignment score.
Since this paper is only the second to formally study concepts of alignment, our alignment metric can likely be improved.
More work should be done to develop a metric for alignment that consistently reflects a controller's ability to keep a system aligned.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.5\textwidth]{img/envC_alignment.png}
%     \caption{The average alignment score for all paths with each controller in Environment C. Interestingly, S2C achieves the best (lowest) alignment score, despite have a very high number of resets and low travel distance between resets. ARC achieves an alignment score lower than APF, but worse than S2C. The reason for this is not clear, since S2C is not designed around alignment. This suggests that measuring alignment score may not be the most useful metric, since ARC is able to achieve much better performance than S2C, but still has a worse alignment score.}
%     \label{fig:envC_alignment}
% \end{figure}

\subsubsection{Qualitative Evaluations}
A heat map of the user in the physical space for Environment C is shown in \autoref{fig:teaser}.
% The black rectangles represent obstacles in the environment, and purple tiles indicate low frequency of the user being in that area, while yellow tiles indicate high frequency.
It is clear that ARC utilizes more of the PE for navigation than do APF or S2C, but there is still a bias towards the leftmost region of the room.
This is similar to the bias seen in the heat map for ARC in Environment B, which suggests that this may not be a product of random chance and that ARC prefers to steer the user to a particular region of the PE.
% We saw a bias in the user's position when using ARC in both Environment B and C, which suggests that there is something going on that is causing ARC to prefer parts of the room over others.
Visual inspection of the random starting positions in the PE confirmed that the bias was not due to the starting position, so more work should be done to get a better understanding of the biases of ARC.

% APF does worse than ARC at using all of the space available in the PE, with the user being concentrated mostly in the open space in the bottom region of the room.
% The user is able to walk through the other regions in the room sometimes, but the algorithm shows a clear bias towards the largest free space in the room.
% S2C performs very poorly, since there is an obstacle in the center of the physical room.
% The user is constantly redirected towards the center, only to be turned away when they get too close, and then steered right back to the center.
% The high concentration near the center of the room is supported by the very high number of resets they incurred in this space (see \autoref{fig:envC_resets}).

The performance of ARC, APF, and S2C is also compared in \autoref{fig:resets_by_CR}.
ARC achieves much fewer resets than either APF or S2C in Environment C, which is the most complex, which highlights ARC's ability to handle physical and virtual environments with differing configurations and complexities.
Interestingly, the performance of ARC increases going from Environment B to Environment C, which suggests that in addition to the complexity metric we used (measure of relative proximity to obstacles in the PE and VE), the shapes of the free space may be important for an algorithm's performance.
% It should also be noted that APF and S2C do not see this same increase in performance from Environment B to C, and both consistently get worse as the complexity increases, as one would expect.
% This shows that our novel complexity metric is still useful for assessing controller performance in complex environments.

Finally, \autoref{fig:envC_steering} shows a frequency plot of the gains applied by each controller across all paths in Environment C.
All gains applied by both ARC and S2C are lower than that of APF, with ARC applying the lowest gains of all, and applying stronger gains less often than S2C.
This highlights one of the major strength of our algorithm: ARC is able to achieve a lower number of resets than current state of the art while also applying \textit{less intense} gains.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/resets_by_CR.png}
    \caption{The relationship between the environment complexity and the number of resets incurred by a redirection controller. ARC consistently has a better performance than S2C and APF for all environment complexities. The performance difference between ARC and the other algorithms is quite large for environments A and C, but the difference decreases drastically for Environment B. It is not clear why Environment B causes the controllers to have a more similar performance, but it may be due to the relatively few pathing options afforded by the narrow hallways of Environment B. Environments A and C both include regions with a fairly large amount of open space, unlike Environment B (see \autoref{fig:environments}).}
    \label{fig:resets_by_CR}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{img/envC_steering_rate_short.png}
    \caption{The average curvature gain applied by each controller for all paths in Environment C. The same trend as in Environment B is seen here, where APF has a higher steering rate than S2C and ARC. One difference between the steering rates in Environment B and C is that the gains applied by S2C and ARC are in a higher range ($6^\circ/s - 7^\circ/s$) in Environment C than they were in Environment B ($4^\circ/s - 6^\circ/s$).}
    \label{fig:envC_steering}
\end{figure}

